The Extraordinary Outburst in the Massive Protostellar System NGC6334I-MM1: Emergence of Strong 6.7 GHz Methanol Masers

We report the first sub-arcsecond VLA imaging of 6 GHz continuum, methanol maser, and excited-state hydroxyl maser emission toward the massive protostellar cluster NGC6334I following the recent 2015 outburst in (sub)millimeter continuum toward MM1, the strongest (sub)millimeter source in the protocluster. In addition to detections toward the previously known 6.7 GHz Class II methanol maser sites in the hot core MM2 and the UCHII region MM3 (NGC6334F), we find new maser features toward several components of MM1, along with weaker features $\sim1''$ north, west, and southwest of MM1, and toward the non-thermal radio continuum source CM2. None of these areas have heretofore exhibited Class II methanol maser emission in three decades of observations. The strongest MM1 masers trace a dust cavity, while no masers are seen toward the strongest dust sources MM1A, 1B and 1D. The locations of the masers are consistent with a combination of increased radiative pumping due to elevated dust grain temperature following the outburst, the presence of infrared photon propagation cavities, and the presence of high methanol column densities as indicated by ALMA images of thermal transitions. The non-thermal radio emission source CM2 ($2''$ north of MM1) also exhibits new maser emission from the excited 6.035 and 6.030 GHz OH lines. Using the Zeeman effect, we measure a line-of-sight magnetic field of +0.5 to +3.7 mG toward CM2. In agreement with previous studies, we also detect numerous methanol and excited OH maser spots toward the UCHII region MM3, with predominantly negative line-of-sight magnetic field strengths of -2 to -5 mG and an intriguing south-north field reversal.

==> ch3oh_table.tex <==
  1 & UCHII-Met4 & -18.80 & 17:20:53.3729 & -35:47:01.474 & 0.0119 (0.0015)\\
  2 & UCHII-Met4 & -18.65 & 17:20:53.3721 & -35:47:01.382 & 0.00893 (0.00148)\\
  3 & UCHII-Met4 & -17.75 & 17:20:53.3703 & -35:47:01.456 & 0.0114 (0.0015)\\
  4 & UCHII-Met4 & -17.60 & 17:20:53.3715 & -35:47:01.356 & 0.0119 (0.0015)\\
  5 & UCHII-Met4 & -17.45 & 17:20:53.3705 & -35:47:01.393 & 0.00988 (0.00147)\\
  6 & UCHII-Met4 & -17.30 & 17:20:53.3696 & -35:47:01.361 & 0.0110 (0.0015)\\
  7 & UCHII-Met4 & -17.15 & 17:20:53.3663 & -35:47:01.416 & 0.0109 (0.0015)\\
  8 & UCHII-Met4 & -17.00 & 17:20:53.3710 & -35:47:01.394 & 0.0111 (0.0015)\\
  9 & UCHII-Met4 & -16.85 & 17:20:53.3685 & -35:47:01.503 & 0.0150 (0.0014)\\
 10 & UCHII-Met4 & -16.70 & 17:20:53.3684 & -35:47:01.496 & 0.0171 (0.0015)\\
 11 & UCHII-Met4 & -16.55 & 17:20:53.3703 & -35:47:01.547 & 0.0173 (0.0015)\\
 12 & UCHII-Met4 & -16.40 & 17:20:53.3711 & -35:47:01.583 & 0.0167 (0.0015)\\
 13 & UCHII-Met4 & -16.25 & 17:20:53.3690 & -35:47:01.514 & 0.0145 (0.0015)\\
 14 & UCHII-Met4 & -16.10 & 17:20:53.3700 & -35:47:01.470 & 0.0169 (0.0015)\\
 15 & MM2-Met1 & -15.95 & 17:20:53.1741 & -35:46:59.098 & 0.0104 (0.0015)\\
 16 & UCHII-Met4 & -15.95 & 17:20:53.3702 & -35:47:01.538 & 0.0207 (0.0015)\\
 17 & MM2-Met1 & -15.80 & 17:20:53.1768 & -35:46:59.247 & 0.00923 (0.00153)\\
 18 & UCHII-Met4 & -15.80 & 17:20:53.3700 & -35:47:01.569 & 0.0198 (0.0015)\\
 19 & MM2-Met1 & -15.65 & 17:20:53.1771 & -35:46:59.230 & 0.00867 (0.00151)\\
 20 & UCHII-Met4 & -15.65 & 17:20:53.3695 & -35:47:01.497 & 0.0235 (0.0015)\\
 21 & UCHII-Met4 & -15.50 & 17:20:53.3689 & -35:47:01.474 & 0.0235 (0.0015)\\
 22 & MM2-Met1 & -15.50 & 17:20:53.1767 & -35:46:59.221 & 0.00792 (0.00146)\\
 23 & MM2-Met1 & -15.35 & 17:20:53.1797 & -35:46:59.243 & 0.0107 (0.0015)\\
 24 & UCHII-Met4 & -15.35 & 17:20:53.3690 & -35:47:01.486 & 0.0255 (0.0015)\\
 25 & MM2-Met1 & -15.20 & 17:20:53.1782 & -35:46:59.128 & 0.0108 (0.0015)\\
 26 & UCHII-Met4 & -15.20 & 17:20:53.3695 & -35:47:01.480 & 0.0277 (0.0015)\\
 27 & MM2-Met1 & -15.05 & 17:20:53.1755 & -35:46:59.278 & 0.0133 (0.0016)\\
 28 & UCHII-Met4 & -15.05 & 17:20:53.3690 & -35:47:01.464 & 0.0274 (0.0016)\\
 29 & MM2-Met1 & -14.90 & 17:20:53.1749 & -35:46:59.217 & 0.0189 (0.0015)\\
 30 & UCHII-Met4 & -14.90 & 17:20:53.3699 & -35:47:01.483 & 0.0314 (0.0015)\\
 31 & UCHII-Met4 & -14.75 & 17:20:53.3703 & -35:47:01.450 & 0.0319 (0.0015)\\
 32 & MM2-Met1 & -14.75 & 17:20:53.1737 & -35:46:59.162 & 0.0197 (0.0015)\\
 33 & MM2-Met1 & -14.60 & 17:20:53.1752 & -35:46:59.167 & 0.0190 (0.0016)\\
 34 & UCHII-Met4 & -14.60 & 17:20:53.3699 & -35:47:01.513 & 0.0328 (0.0016)\\
 35 & MM2-Met1 & -14.45 & 17:20:53.1761 & -35:46:59.192 & 0.0193 (0.0015)\\
 36 & UCHII-Met4 & -14.45 & 17:20:53.3693 & -35:47:01.525 & 0.0404 (0.0015)\\
 37 & MM2-Met1 & -14.30 & 17:20:53.1750 & -35:46:59.137 & 0.0215 (0.0015)\\
 38 & UCHII-Met4 & -14.30 & 17:20:53.3693 & -35:47:01.504 & 0.0406 (0.0015)\\
 39 & UCHII-Met4 & -14.15 & 17:20:53.3684 & -35:47:01.529 & 0.0450 (0.0016)\\
 40 & MM2-Met1 & -14.15 & 17:20:53.1754 & -35:46:59.158 & 0.0236 (0.0016)\\
 41 & UCHII-Met4 & -14.00 & 17:20:53.3686 & -35:47:01.517 & 0.0494 (0.0016)\\
 42 & MM2-Met1 & -14.00 & 17:20:53.1761 & -35:46:59.137 & 0.0235 (0.0016)\\
 43 & MM2-Met1 & -13.85 & 17:20:53.1761 & -35:46:59.152 & 0.0283 (0.0016)\\
 44 & UCHII-Met4 & -13.85 & 17:20:53.3688 & -35:47:01.533 & 0.0514 (0.0016)\\
 45 & MM2-Met1 & -13.70 & 17:20:53.1760 & -35:46:59.153 & 0.0351 (0.0016)\\
 46 & UCHII-Met4 & -13.70 & 17:20:53.3575 & -35:47:01.922 & 0.0145 (0.0016)\\
 47 & UCHII-Met4 & -13.70 & 17:20:53.3700 & -35:47:01.474 & 0.0552 (0.0016)\\
 48 & MM2-Met1 & -13.55 & 17:20:53.1759 & -35:46:59.163 & 0.0384 (0.0016)\\
 49 & UCHII-Met4 & -13.55 & 17:20:53.3609 & -35:47:01.847 & 0.0175 (0.0016)\\
 50 & UCHII-Met4 & -13.55 & 17:20:53.3707 & -35:47:01.455 & 0.0604 (0.0016)\\
 51 & UCHII-Met4 & -13.40 & 17:20:53.3718 & -35:47:01.472 & 0.0598 (0.0016)\\
 52 & MM2-Met1 & -13.40 & 17:20:53.1760 & -35:46:59.165 & 0.0451 (0.0016)\\
 53 & UCHII-Met4 & -13.40 & 17:20:53.3624 & -35:47:01.782 & 0.0248 (0.0016)\\
 54 & MM2-Met1 & -13.25 & 17:20:53.1754 & -35:46:59.168 & 0.0475 (0.0016)\\
 55 & UCHII-Met4 & -13.25 & 17:20:53.3589 & -35:47:01.846 & 0.0196 (0.0016)\\
 56 & UCHII-Met4 & -13.25 & 17:20:53.3706 & -35:47:01.495 & 0.0727 (0.0016)\\
 57 & MM2-Met1 & -13.10 & 17:20:53.1755 & -35:46:59.170 & 0.0545 (0.0017)\\
 58 & UCHII-Met4 & -13.10 & 17:20:53.3686 & -35:47:01.533 & 0.0883 (0.0017)\\
 59 & MM2-Met1 & -12.95 & 17:20:53.1763 & -35:46:59.171 & 0.0654 (0.0016)\\
 60 & UCHII-Met4 & -12.95 & 17:20:53.3693 & -35:47:01.520 & 0.104 (0.002)\\
 61 & UCHII-Met4 & -12.80 & 17:20:53.3695 & -35:47:01.517 & 0.121 (0.002)\\
 62 & MM2-Met1 & -12.80 & 17:20:53.1766 & -35:46:59.176 & 0.0793 (0.0016)\\
 63 & MM2-Met1 & -12.65 & 17:20:53.1347 & -35:46:59.309 & 0.0214 (0.0017)\\
 64 & MM2-Met1 & -12.65 & 17:20:53.1767 & -35:46:59.184 & 0.0978 (0.0017)\\
 65 & UCHII-Met4 & -12.65 & 17:20:53.3598 & -35:47:01.732 & 0.0488 (0.0017)\\
 66 & UCHII-Met4 & -12.65 & 17:20:53.3715 & -35:47:01.453 & 0.110 (0.002)\\
 67 & MM2-Met1 & -12.50 & 17:20:53.1354 & -35:46:59.309 & 0.0370 (0.0019)\\
 68 & MM2-Met1 & -12.50 & 17:20:53.1769 & -35:46:59.178 & 0.128 (0.002)\\
 69 & UCHII-Met4 & -12.50 & 17:20:53.3603 & -35:47:01.781 & 0.0584 (0.0019)\\
 70 & UCHII-Met4 & -12.50 & 17:20:53.3711 & -35:47:01.446 & 0.137 (0.002)\\
 71 & MM2-Met1 & -12.35 & 17:20:53.1733 & -35:46:59.207 & 0.0937 (0.0019)\\
 72 & UCHII-Met4 & -12.35 & 17:20:53.3711 & -35:47:01.435 & 0.158 (0.002)\\
 73 & UCHII-Met4 & -12.35 & 17:20:53.3607 & -35:47:01.763 & 0.0724 (0.0019)\\
 74 & MM2-Met1 & -12.35 & 17:20:53.1383 & -35:46:59.346 & 0.0463 (0.0019)\\
 75 & MM2-Met1 & -12.35 & 17:20:53.1829 & -35:46:59.122 & 0.106 (0.002)\\
 76 & UCHII-Met4 & -12.20 & 17:20:53.3605 & -35:47:01.744 & 0.100 (0.002)\\
 77 & MM2-Met1 & -12.20 & 17:20:53.1433 & -35:46:59.292 & 0.269 (0.002)\\
 78 & MM2-Met1 & -12.20 & 17:20:53.1736 & -35:46:59.192 & 0.155 (0.002)\\
 79 & MM2-Met1 & -12.20 & 17:20:53.1861 & -35:46:59.140 & 0.205 (0.002)\\
 80 & UCHII-Met4 & -12.20 & 17:20:53.3715 & -35:47:01.418 & 0.194 (0.002)\\
 81 & UCHII-Met4 & -12.05 & 17:20:53.3717 & -35:47:01.397 & 0.275 (0.002)\\
 82 & UCHII-Met4 & -12.05 & 17:20:53.3603 & -35:47:01.741 & 0.137 (0.002)\\
 83 & MM2-Met1 & -12.05 & 17:20:53.1443 & -35:46:59.287 & 1.21 (0.01)\\
 84 & MM2-Met1 & -12.05 & 17:20:53.1725 & -35:46:59.195 & 0.284 (0.002)\\
 85 & MM2-Met1 & -12.05 & 17:20:53.1869 & -35:46:59.148 & 0.461 (0.002)\\
 86 & MM2-Met1 & -11.90 & 17:20:53.1447 & -35:46:59.286 & 2.15 (0.01)\\
 87 & MM2-Met1 & -11.90 & 17:20:53.1715 & -35:46:59.211 & 0.969 (0.002)\\
 88 & MM2-Met1 & -11.90 & 17:20:53.1868 & -35:46:59.154 & 1.17 (0.01)\\
 89 & UCHII-Met4 & -11.90 & 17:20:53.3595 & -35:47:01.753 & 0.200 (0.002)\\
 90 & UCHII-Met4 & -11.90 & 17:20:53.3719 & -35:47:01.366 & 0.667 (0.002)\\
 91 & MM2-Met1 & -11.75 & 17:20:53.1447 & -35:46:59.290 & 1.59 (0.01)\\
 92 & MM2-Met1 & -11.75 & 17:20:53.1671 & -35:46:59.231 & 3.27 (0.01)\\
 93 & MM2-Met1 & -11.75 & 17:20:53.1770 & -35:46:59.191 & 4.33 (0.01)\\
 94 & MM2-Met1 & -11.75 & 17:20:53.1881 & -35:46:59.153 & 2.79 (0.01)\\
 95 & UCHII-Met4 & -11.75 & 17:20:53.3588 & -35:47:01.761 & 0.358 (0.003)\\
 96 & UCHII-Met4 & -11.75 & 17:20:53.3719 & -35:47:01.361 & 1.11 (0.01)\\
 97 & UCHII-Met4 & -11.60 & 17:20:53.3718 & -35:47:01.357 & 1.37 (0.02)\\
 98 & MM2-Met1 & -11.60 & 17:20:53.1856 & -35:46:59.151 & 13.4 (0.1)\\
 99 & UCHII-Met4 & -11.60 & 17:20:53.3573 & -35:47:01.773 & 2.56 (0.02)\\
100 & MM2-Met1 & -11.60 & 17:20:53.1668 & -35:46:59.236 & 16.2 (0.1)\\
101 & MM2-Met1 & -11.60 & 17:20:53.1446 & -35:46:59.356 & 0.860 (0.017)\\
102 & MM2-Met1 & -11.60 & 17:20:53.1772 & -35:46:59.184 & 28.6 (0.1)\\
103 & MM2-Met1 & -11.45 & 17:20:53.1664 & -35:46:59.244 & 38.2 (0.1)\\
104 & MM2-Met1 & -11.45 & 17:20:53.1768 & -35:46:59.172 & 127 (1)\\
105 & MM2-Met1 & -11.45 & 17:20:53.1825 & -35:46:59.170 & 104 (1)\\
106 & UCHII-Met4 & -11.45 & 17:20:53.3568 & -35:47:01.764 & 43.1 (0.1)\\
107 & UCHII-Met4 & -11.45 & 17:20:53.3717 & -35:47:01.389 & 2.85 (0.05)\\
108 & UCHII-Met4 & -11.30 & 17:20:53.3692 & -35:47:01.474 & 8.66 (0.09)\\
109 & UCHII-Met4 & -11.30 & 17:20:53.3566 & -35:47:01.765 & 247 (1)\\
110 & MM2-Met1 & -11.30 & 17:20:53.1758 & -35:46:59.165 & 278 (1)\\
111 & MM2-Met1 & -11.30 & 17:20:53.1663 & -35:46:59.253 & 49.5 (0.1)\\
112 & MM2-Met1 & -11.30 & 17:20:53.1805 & -35:46:59.174 & 400 (1)\\
113 & MM2-Met1 & -11.15 & 17:20:53.1660 & -35:46:59.270 & 37.4 (0.2)\\
114 & MM2-Met1 & -11.15 & 17:20:53.1753 & -35:46:59.161 & 426 (1)\\
115 & MM2-Met1 & -11.15 & 17:20:53.1796 & -35:46:59.179 & 583 (1)\\
116 & UCHII-Met4 & -11.15 & 17:20:53.3562 & -35:47:01.764 & 383 (1)\\
117 & UCHII-Met4 & -11.15 & 17:20:53.3666 & -35:47:01.603 & 34.6 (0.2)\\
118 & UCHII-Met4 & -11.00 & 17:20:53.3697 & -35:47:01.402 & 30.8 (0.1)\\
119 & UCHII-Met4 & -11.00 & 17:20:53.3542 & -35:47:01.747 & 151 (1)\\
120 & UCHII-Met4 & -11.00 & 17:20:53.3615 & -35:47:01.779 & 145 (1)\\
121 & MM2-Met1 & -11.00 & 17:20:53.1782 & -35:46:59.171 & 580 (1)\\
122 & MM1-Met2 & -11.00 & 17:20:53.3342 & -35:46:58.598 & 3.81 (0.10)\\
123 & MM2-Met1 & -11.00 & 17:20:53.1719 & -35:46:59.177 & 143 (1)\\
124 & MM2-Met1 & -10.85 & 17:20:53.1694 & -35:46:59.177 & 60.1 (0.1)\\
125 & MM2-Met1 & -10.85 & 17:20:53.1777 & -35:46:59.171 & 205 (1)\\
126 & MM1-Met2 & -10.85 & 17:20:53.3341 & -35:46:58.579 & 4.73 (0.09)\\
127 & UCHII-Met4 & -10.85 & 17:20:53.3561 & -35:47:01.762 & 93.6 (0.1)\\
128 & UCHII-Met4 & -10.85 & 17:20:53.3654 & -35:47:01.900 & 126 (1)\\
129 & UCHII-Met4 & -10.85 & 17:20:53.3699 & -35:47:01.518 & 118 (1)\\
130 & MM1-Met2 & -10.70 & 17:20:53.3346 & -35:46:58.627 & 2.82 (0.11)\\
131 & UCHII-Met4 & -10.70 & 17:20:53.3700 & -35:47:01.496 & 575 (1)\\
132 & UCHII-Met4 & -10.70 & 17:20:53.3680 & -35:47:01.848 & 180 (1)\\
133 & MM2-Met1 & -10.70 & 17:20:53.1761 & -35:46:59.167 & 76.1 (0.1)\\
134 & MM2-Met1 & -10.70 & 17:20:53.1654 & -35:46:59.192 & 54.3 (0.1)\\
135 & UCHII-Met4 & -10.70 & 17:20:53.3594 & -35:47:01.815 & 58.9 (0.1)\\
136 & MM2-Met1 & -10.55 & 17:20:53.1639 & -35:46:59.196 & 72.8 (0.1)\\
137 & MM2-Met1 & -10.55 & 17:20:53.1744 & -35:46:59.169 & 39.3 (0.1)\\
138 & UCHII-Met4 & -10.55 & 17:20:53.3671 & -35:47:01.721 & 410 (1)\\
139 & UCHII-Met4 & -10.55 & 17:20:53.3704 & -35:47:01.474 & 1510 (1)\\
140 & UCHII-Met4 & -10.40 & 17:20:53.3678 & -35:47:01.604 & 1270 (1)\\
141 & UCHII-Met4 & -10.40 & 17:20:53.3718 & -35:47:01.423 & 1820 (1)\\
142 & MM2-Met1 & -10.40 & 17:20:53.1735 & -35:46:59.174 & 29.3 (0.4)\\
143 & MM2-Met1 & -10.40 & 17:20:53.1632 & -35:46:59.192 & 93.3 (0.4)\\
144 & MM2-Met1 & -10.25 & 17:20:53.1618 & -35:46:59.182 & 133 (1)\\
145 & MM2-Met1 & -10.25 & 17:20:53.1705 & -35:46:59.177 & 49.8 (0.3)\\
146 & MM1-Met2 & -10.25 & 17:20:53.3307 & -35:46:58.054 & 4.08 (0.30)\\
147 & UCHII-Met4 & -10.25 & 17:20:53.3683 & -35:47:01.566 & 1180 (1)\\
148 & UCHII-Met4 & -10.25 & 17:20:53.3728 & -35:47:01.400 & 1130 (1)\\
149 & UCHII-Met7 & -10.25 & 17:20:53.4530 & -35:47:00.534 & 23.8 (0.3)\\
150 & MM1-Met2 & -10.10 & 17:20:53.3322 & -35:46:58.296 & 3.44 (0.15)\\
151 & MM2-Met1 & -10.10 & 17:20:53.1616 & -35:46:59.176 & 174 (1)\\
152 & MM2-Met1 & -10.10 & 17:20:53.1726 & -35:46:59.177 & 48.1 (0.2)\\
153 & UCHII-Met4 & -10.10 & 17:20:53.3682 & -35:47:01.574 & 301 (1)\\
154 & UCHII-Met4 & -10.10 & 17:20:53.3733 & -35:47:01.402 & 420 (1)\\
155 & UCHII-Met6 & -10.10 & 17:20:53.3831 & -35:47:01.004 & 16.9 (0.2)\\
156 & UCHII-Met7 & -10.10 & 17:20:53.4529 & -35:47:00.503 & 36.3 (0.2)\\
157 & UCHII-Met6 &  -9.95 & 17:20:53.3843 & -35:47:00.967 & 10.7 (0.1)\\
158 & UCHII-Met4 &  -9.95 & 17:20:53.3765 & -35:47:01.397 & 133 (1)\\
159 & UCHII-Met7 &  -9.95 & 17:20:53.4537 & -35:47:00.485 & 33.5 (0.1)\\
160 & UCHII-Met7 &  -9.95 & 17:20:53.4457 & -35:47:00.596 & 9.28 (0.10)\\
161 & UCHII-Met4 &  -9.95 & 17:20:53.3707 & -35:47:01.458 & 90.5 (0.1)\\
162 & MM1-Met2 &  -9.95 & 17:20:53.3204 & -35:46:58.133 & 1.39 (0.10)\\
163 & MM1-Met2 &  -9.95 & 17:20:53.3405 & -35:46:58.730 & 2.55 (0.10)\\
164 & MM2-Met1 &  -9.95 & 17:20:53.2046 & -35:46:58.931 & 2.33 (0.10)\\
165 & MM2-Met1 &  -9.95 & 17:20:53.1786 & -35:46:59.139 & 24.6 (0.1)\\
166 & MM2-Met1 &  -9.95 & 17:20:53.1659 & -35:46:59.181 & 70.9 (0.1)\\
167 & MM2-Met1 &  -9.95 & 17:20:53.1592 & -35:46:59.169 & 68.7 (0.1)\\
168 & UCHII-Met7 &  -9.80 & 17:20:53.4536 & -35:47:00.485 & 15.1 (0.1)\\
169 & UCHII-Met7 &  -9.80 & 17:20:53.4450 & -35:47:00.628 & 13.5 (0.1)\\
170 & UCHII-Met4 &  -9.80 & 17:20:53.3847 & -35:47:01.427 & 60.1 (0.1)\\
171 & UCHII-Met4 &  -9.80 & 17:20:53.3748 & -35:47:01.408 & 461 (1)\\
172 & MM1-Met2 &  -9.80 & 17:20:53.3106 & -35:46:58.142 & 3.98 (0.08)\\
173 & MM2-Met1 &  -9.80 & 17:20:53.2030 & -35:46:58.946 & 4.24 (0.08)\\
174 & MM2-Met1 &  -9.80 & 17:20:53.1763 & -35:46:59.146 & 22.6 (0.1)\\
175 & MM2-Met1 &  -9.80 & 17:20:53.1612 & -35:46:59.170 & 49.0 (0.1)\\
176 & MM1-Met2 &  -9.80 & 17:20:53.3389 & -35:46:58.780 & 3.98 (0.08)\\
177 & UCHII-Met4 &  -9.65 & 17:20:53.3876 & -35:47:01.383 & 81.1 (0.1)\\
178 & UCHII-Met7 &  -9.65 & 17:20:53.4459 & -35:47:00.607 & 15.0 (0.1)\\
179 & MM1-Met2 &  -9.65 & 17:20:53.3396 & -35:46:58.797 & 8.16 (0.09)\\
180 & UCHII-Met4 &  -9.65 & 17:20:53.3749 & -35:47:01.407 & 478 (1)\\
181 & MM2-Met1 &  -9.65 & 17:20:53.2017 & -35:46:58.919 & 3.39 (0.09)\\
182 & MM2-Met1 &  -9.65 & 17:20:53.1740 & -35:46:59.143 & 8.95 (0.09)\\
183 & MM2-Met1 &  -9.65 & 17:20:53.1572 & -35:46:59.133 & 15.6 (0.1)\\
184 & MM1-Met2 &  -9.65 & 17:20:53.3129 & -35:46:58.054 & 8.51 (0.09)\\
185 & UCHII-Met7 &  -9.50 & 17:20:53.4450 & -35:47:00.619 & 6.16 (0.07)\\
186 & UCHII-Met5 &  -9.50 & 17:20:53.4145 & -35:47:01.435 & 2.74 (0.07)\\
187 & UCHII-Met4 &  -9.50 & 17:20:53.3878 & -35:47:01.361 & 61.7 (0.1)\\
188 & UCHII-Met4 &  -9.50 & 17:20:53.3752 & -35:47:01.411 & 67.9 (0.1)\\
189 & MM1-Met2 &  -9.50 & 17:20:53.3202 & -35:46:57.894 & 28.2 (0.1)\\
190 & MM1-Met2 &  -9.50 & 17:20:53.3398 & -35:46:58.816 & 10.5 (0.1)\\
191 & MM2-Met1 &  -9.50 & 17:20:53.1979 & -35:46:58.835 & 1.53 (0.07)\\
192 & MM2-Met1 &  -9.50 & 17:20:53.1757 & -35:46:59.074 & 2.33 (0.07)\\
193 & MM2-Met1 &  -9.50 & 17:20:53.1577 & -35:46:59.192 & 6.36 (0.07)\\
194 & MM2-Met1 &  -9.50 & 17:20:53.1476 & -35:46:58.943 & 10.7 (0.1)\\
195 & MM1-Met2 &  -9.50 & 17:20:53.3102 & -35:46:58.095 & 5.58 (0.07)\\
196 & UCHII-Met4 &  -9.35 & 17:20:53.3884 & -35:47:01.398 & 9.47 (0.02)\\
197 & UCHII-Met7 &  -9.35 & 17:20:53.4443 & -35:47:00.604 & 1.41 (0.02)\\
198 & UCHII-Met5 &  -9.35 & 17:20:53.4317 & -35:47:01.433 & 2.33 (0.02)\\
199 & UCHII-Met1 &  -9.35 & 17:20:53.4195 & -35:47:03.221 & 2.40 (0.02)\\
200 & UCHII-Met5 &  -9.35 & 17:20:53.4107 & -35:47:01.508 & 3.35 (0.02)\\
201 & UCHII-Met2 &  -9.35 & 17:20:53.3979 & -35:47:02.605 & 1.21 (0.02)\\
202 & UCHII-Met4 &  -9.35 & 17:20:53.3791 & -35:47:01.421 & 9.73 (0.02)\\
203 & MM1-Met2 &  -9.35 & 17:20:53.3395 & -35:46:58.811 & 6.03 (0.02)\\
204 & MM1-Met2 &  -9.35 & 17:20:53.3201 & -35:46:57.899 & 55.4 (0.1)\\
205 & MM1-Met2 &  -9.35 & 17:20:53.3083 & -35:46:58.066 & 1.90 (0.02)\\
206 & MM2-Met1 &  -9.35 & 17:20:53.1876 & -35:46:58.925 & 0.982 (0.021)\\
207 & MM2-Met1 &  -9.35 & 17:20:53.1626 & -35:46:59.148 & 2.90 (0.02)\\
208 & MM2-Met1 &  -9.35 & 17:20:53.1505 & -35:46:59.149 & 10.8 (0.1)\\
209 & MM2-Met1 &  -9.35 & 17:20:53.1469 & -35:46:58.885 & 9.63 (0.02)\\
210 & UCHII-Met5 &  -9.20 & 17:20:53.4335 & -35:47:01.459 & 5.03 (0.02)\\
211 & UCHII-Met1 &  -9.20 & 17:20:53.4194 & -35:47:03.213 & 3.01 (0.02)\\
212 & UCHII-Met5 &  -9.20 & 17:20:53.4131 & -35:47:01.416 & 3.19 (0.02)\\
213 & UCHII-Met5 &  -9.20 & 17:20:53.3990 & -35:47:01.646 & 2.29 (0.02)\\
214 & UCHII-Met2 &  -9.20 & 17:20:53.3974 & -35:47:02.648 & 2.57 (0.02)\\
215 & UCHII-Met4 &  -9.20 & 17:20:53.3794 & -35:47:01.417 & 6.00 (0.02)\\
216 & UCHII-Met7 &  -9.20 & 17:20:53.4431 & -35:47:00.602 & 0.486 (0.022)\\
217 & MM1-Met2 &  -9.20 & 17:20:53.3198 & -35:46:57.901 & 40.5 (0.1)\\
218 & MM1-Met2 &  -9.20 & 17:20:53.3037 & -35:46:58.300 & 0.740 (0.022)\\
219 & MM2-Met1 &  -9.20 & 17:20:53.1876 & -35:46:58.972 & 0.562 (0.022)\\
220 & MM2-Met1 &  -9.20 & 17:20:53.1587 & -35:46:59.157 & 3.88 (0.02)\\
221 & MM2-Met1 &  -9.20 & 17:20:53.1488 & -35:46:59.137 & 16.8 (0.1)\\
222 & MM2-Met1 &  -9.20 & 17:20:53.1470 & -35:46:58.858 & 5.37 (0.02)\\
223 & MM1-Met2 &  -9.20 & 17:20:53.3390 & -35:46:58.735 & 3.56 (0.02)\\
224 & UCHII-Met7 &  -9.05 & 17:20:53.4411 & -35:47:00.629 & 0.260 (0.031)\\
225 & UCHII-Met5 &  -9.05 & 17:20:53.4336 & -35:47:01.467 & 9.07 (0.03)\\
226 & UCHII-Met1 &  -9.05 & 17:20:53.4177 & -35:47:03.088 & 1.49 (0.03)\\
227 & UCHII-Met5 &  -9.05 & 17:20:53.4135 & -35:47:01.383 & 3.91 (0.03)\\
228 & UCHII-Met5 &  -9.05 & 17:20:53.3985 & -35:47:01.582 & 2.48 (0.03)\\
229 & UCHII-Met2 &  -9.05 & 17:20:53.3984 & -35:47:02.634 & 4.57 (0.03)\\
230 & UCHII-Met4 &  -9.05 & 17:20:53.3833 & -35:47:01.386 & 7.50 (0.03)\\
231 & MM1-Met2 &  -9.05 & 17:20:53.3191 & -35:46:57.893 & 46.7 (0.1)\\
232 & MM1-Met2 &  -9.05 & 17:20:53.3013 & -35:46:58.300 & 0.647 (0.031)\\
233 & MM2-Met1 &  -9.05 & 17:20:53.1645 & -35:46:59.200 & 1.58 (0.03)\\
234 & MM2-Met1 &  -9.05 & 17:20:53.1487 & -35:46:59.107 & 20.9 (0.1)\\
235 & MM1-Met2 &  -9.05 & 17:20:53.3383 & -35:46:58.499 & 3.51 (0.03)\\
236 & UCHII-Met5 &  -8.90 & 17:20:53.3969 & -35:47:01.560 & 2.06 (0.03)\\
237 & UCHII-Met5 &  -8.90 & 17:20:53.4334 & -35:47:01.486 & 13.9 (0.1)\\
238 & UCHII-Met2 &  -8.90 & 17:20:53.4155 & -35:47:02.879 & 2.14 (0.03)\\
239 & UCHII-Met5 &  -8.90 & 17:20:53.4137 & -35:47:01.414 & 4.28 (0.03)\\
240 & UCHII-Met6 &  -8.90 & 17:20:53.4028 & -35:47:00.600 & 0.811 (0.029)\\
241 & UCHII-Met2 &  -8.90 & 17:20:53.4001 & -35:47:02.624 & 3.68 (0.03)\\
242 & UCHII-Met4 &  -8.90 & 17:20:53.3846 & -35:47:01.388 & 16.7 (0.1)\\
243 & MM1-Met2 &  -8.90 & 17:20:53.3190 & -35:46:57.871 & 41.3 (0.1)\\
244 & MM1-Met2 &  -8.90 & 17:20:53.3379 & -35:46:58.369 & 4.32 (0.03)\\
245 & MM1-Met2 &  -8.90 & 17:20:53.3699 & -35:46:58.700 & 0.845 (0.029)\\
246 & MM1-Met2 &  -8.90 & 17:20:53.3000 & -35:46:57.998 & 1.04 (0.03)\\
247 & MM2-Met1 &  -8.90 & 17:20:53.1645 & -35:46:59.200 & 0.977 (0.029)\\
248 & MM2-Met1 &  -8.90 & 17:20:53.1477 & -35:46:59.113 & 12.5 (0.1)\\
249 & UCHII-Met5 &  -8.75 & 17:20:53.4281 & -35:47:01.382 & 3.74 (0.02)\\
250 & UCHII-Met2 &  -8.75 & 17:20:53.4154 & -35:47:02.871 & 3.03 (0.02)\\
251 & UCHII-Met5 &  -8.75 & 17:20:53.4110 & -35:47:01.471 & 2.84 (0.02)\\
252 & UCHII-Met6 &  -8.75 & 17:20:53.4028 & -35:47:00.600 & 1.09 (0.02)\\
253 & UCHII-Met2 &  -8.75 & 17:20:53.4017 & -35:47:02.595 & 1.55 (0.02)\\
254 & UCHII-Met4 &  -8.75 & 17:20:53.3874 & -35:47:01.418 & 3.99 (0.02)\\
255 & UCHII-Met4 &  -8.75 & 17:20:53.3795 & -35:47:01.360 & 1.99 (0.02)\\
256 & UCHII-Met5 &  -8.75 & 17:20:53.4344 & -35:47:01.523 & 38.0 (0.1)\\
257 & MM1-Met2 &  -8.75 & 17:20:53.3400 & -35:46:58.428 & 2.39 (0.02)\\
258 & MM1-Met2 &  -8.75 & 17:20:53.3293 & -35:46:57.839 & 5.33 (0.02)\\
259 & MM1-Met2 &  -8.75 & 17:20:53.3187 & -35:46:57.838 & 28.2 (0.1)\\
260 & MM1-Met2 &  -8.75 & 17:20:53.3042 & -35:46:57.976 & 1.23 (0.02)\\
261 & MM2-Met1 &  -8.75 & 17:20:53.1645 & -35:46:59.200 & 0.686 (0.024)\\
262 & MM2-Met1 &  -8.75 & 17:20:53.1462 & -35:46:59.120 & 6.39 (0.02)\\
263 & MM1-Met2 &  -8.75 & 17:20:53.3699 & -35:46:58.700 & 2.02 (0.02)\\
264 & UCHII-Met5 &  -8.60 & 17:20:53.4347 & -35:47:01.525 & 88.9 (0.1)\\
265 & MM1-Met1 &  -8.60 & 17:20:53.4168 & -35:46:57.031 & 0.202 (0.023)\\
266 & UCHII-Met2 &  -8.60 & 17:20:53.4138 & -35:47:02.788 & 4.78 (0.02)\\
267 & UCHII-Met5 &  -8.60 & 17:20:53.4113 & -35:47:01.461 & 2.68 (0.02)\\
268 & UCHII-Met6 &  -8.60 & 17:20:53.4035 & -35:47:00.670 & 2.08 (0.02)\\
269 & MM1-Met1 &  -8.60 & 17:20:53.3734 & -35:46:56.616 & 0.732 (0.023)\\
270 & MM1-Met2 &  -8.60 & 17:20:53.3567 & -35:46:58.340 & 1.03 (0.02)\\
271 & MM1-Met2 &  -8.60 & 17:20:53.3371 & -35:46:57.784 & 3.96 (0.02)\\
272 & MM1-Met2 &  -8.60 & 17:20:53.3235 & -35:46:57.825 & 14.6 (0.1)\\
273 & MM1-Met2 &  -8.60 & 17:20:53.3155 & -35:46:57.844 & 14.7 (0.1)\\
274 & MM2-Met1 &  -8.60 & 17:20:53.1584 & -35:46:59.303 & 0.971 (0.023)\\
275 & MM2-Met1 &  -8.60 & 17:20:53.1438 & -35:46:59.111 & 2.91 (0.02)\\
276 & MM1-Met2 &  -8.60 & 17:20:53.3724 & -35:46:58.834 & 5.07 (0.02)\\
277 & UCHII-Met1 &  -8.45 & 17:20:53.4084 & -35:47:03.298 & 1.11 (0.02)\\
278 & MM1-Met1 &  -8.45 & 17:20:53.4159 & -35:46:57.037 & 0.613 (0.020)\\
279 & UCHII-Met2 &  -8.45 & 17:20:53.4131 & -35:47:02.655 & 5.47 (0.02)\\
280 & UCHII-Met5 &  -8.45 & 17:20:53.4349 & -35:47:01.528 & 75.8 (0.1)\\
281 & UCHII-Met5 &  -8.45 & 17:20:53.4103 & -35:47:01.417 & 3.63 (0.02)\\
282 & UCHII-Met6 &  -8.45 & 17:20:53.4021 & -35:47:00.763 & 3.15 (0.02)\\
283 & MM1-Met2 &  -8.45 & 17:20:53.3171 & -35:46:57.847 & 13.0 (0.1)\\
284 & MM1-Met2 &  -8.45 & 17:20:53.3719 & -35:46:58.822 & 7.06 (0.02)\\
285 & MM1-Met2 &  -8.45 & 17:20:53.3459 & -35:46:57.786 & 3.04 (0.02)\\
286 & MM1-Met2 &  -8.45 & 17:20:53.3295 & -35:46:57.780 & 7.94 (0.02)\\
287 & MM2-Met1 &  -8.45 & 17:20:53.1614 & -35:46:59.338 & 1.02 (0.02)\\
288 & MM2-Met1 &  -8.45 & 17:20:53.1435 & -35:46:59.130 & 1.40 (0.02)\\
289 & MM1-Met1 &  -8.45 & 17:20:53.3738 & -35:46:56.627 & 0.630 (0.020)\\
290 & UCHII-Met6 &  -8.30 & 17:20:53.3955 & -35:47:01.068 & 1.12 (0.01)\\
291 & MM1-Met1 &  -8.30 & 17:20:53.4026 & -35:46:57.077 & 0.410 (0.012)\\
292 & UCHII-Met6 &  -8.30 & 17:20:53.4033 & -35:47:00.243 & 0.540 (0.012)\\
293 & UCHII-Met6 &  -8.30 & 17:20:53.4054 & -35:47:00.936 & 1.61 (0.01)\\
294 & UCHII-Met2 &  -8.30 & 17:20:53.4128 & -35:47:02.626 & 7.77 (0.01)\\
295 & UCHII-Met5 &  -8.30 & 17:20:53.4094 & -35:47:01.457 & 3.68 (0.01)\\
296 & MM1-Met1 &  -8.30 & 17:20:53.4175 & -35:46:57.019 & 1.85 (0.01)\\
297 & UCHII-Met5 &  -8.30 & 17:20:53.4219 & -35:47:01.348 & 2.39 (0.01)\\
298 & UCHII-Met5 &  -8.30 & 17:20:53.4353 & -35:47:01.534 & 24.8 (0.1)\\
299 & UCHII-Met1 &  -8.30 & 17:20:53.4081 & -35:47:03.309 & 1.40 (0.01)\\
300 & MM1-MetC &  -8.30 & 17:20:53.3807 & -35:46:58.431 & 0.317 (0.012)\\
301 & MM1-Met2 &  -8.30 & 17:20:53.3732 & -35:46:58.872 & 3.15 (0.01)\\
302 & MM1-Met2 &  -8.30 & 17:20:53.3635 & -35:46:58.529 & 0.919 (0.012)\\
303 & MM1-Met2 &  -8.30 & 17:20:53.3455 & -35:46:57.754 & 3.67 (0.01)\\
304 & MM1-Met2 &  -8.30 & 17:20:53.3310 & -35:46:57.767 & 4.39 (0.01)\\
305 & MM1-Met2 &  -8.30 & 17:20:53.3183 & -35:46:57.840 & 4.40 (0.01)\\
306 & MM1-Met2 &  -8.30 & 17:20:53.3000 & -35:46:57.957 & 0.408 (0.012)\\
307 & MM2-Met1 &  -8.30 & 17:20:53.1899 & -35:46:58.876 & 0.333 (0.012)\\
308 & MM2-Met1 &  -8.30 & 17:20:53.1617 & -35:46:59.337 & 1.78 (0.01)\\
309 & MM2-Met1 &  -8.30 & 17:20:53.1471 & -35:46:59.240 & 0.671 (0.012)\\
310 & MM2-Met2 &  -8.30 & 17:20:53.1318 & -35:46:58.722 & 0.448 (0.012)\\
311 & MM1-Met1 &  -8.30 & 17:20:53.3768 & -35:46:56.674 & 0.200 (0.012)\\
312 & UCHII-Met1 &  -8.15 & 17:20:53.4079 & -35:47:03.334 & 1.20 (0.01)\\
313 & UCHII-Met6 &  -8.15 & 17:20:53.4039 & -35:47:00.039 & 0.366 (0.008)\\
314 & UCHII-Met3 &  -8.15 & 17:20:53.4056 & -35:47:01.934 & 0.649 (0.008)\\
315 & UCHII-Met5 &  -8.15 & 17:20:53.4125 & -35:47:01.365 & 3.57 (0.01)\\
316 & UCHII-Met5 &  -8.15 & 17:20:53.4014 & -35:47:01.188 & 1.17 (0.01)\\
317 & MM1-Met1 &  -8.15 & 17:20:53.4145 & -35:46:56.991 & 3.86 (0.01)\\
318 & MM1-Met1 &  -8.15 & 17:20:53.4216 & -35:46:57.040 & 3.54 (0.01)\\
319 & UCHII-Met5 &  -8.15 & 17:20:53.4355 & -35:47:01.534 & 16.6 (0.1)\\
320 & UCHII-Met2 &  -8.15 & 17:20:53.4131 & -35:47:02.633 & 9.07 (0.01)\\
321 & MM1-MetC &  -8.15 & 17:20:53.3829 & -35:46:58.352 & 0.280 (0.008)\\
322 & MM1-Met1 &  -8.15 & 17:20:53.3955 & -35:46:57.143 & 0.459 (0.008)\\
323 & UCHII-Met4 &  -8.15 & 17:20:53.3720 & -35:47:01.449 & 0.164 (0.008)\\
324 & MM2-Met2 &  -8.15 & 17:20:53.1296 & -35:46:58.582 & 1.51 (0.01)\\
325 & MM2-Met1 &  -8.15 & 17:20:53.1599 & -35:46:59.345 & 3.68 (0.01)\\
326 & MM2-Met1 &  -8.15 & 17:20:53.1890 & -35:46:58.861 & 0.594 (0.008)\\
327 & MM1-Met2 &  -8.15 & 17:20:53.2918 & -35:46:57.950 & 0.267 (0.008)\\
328 & MM2-Met1 &  -8.15 & 17:20:53.1479 & -35:46:59.269 & 0.597 (0.008)\\
329 & MM1-Met2 &  -8.15 & 17:20:53.3316 & -35:46:57.753 & 1.79 (0.01)\\
330 & MM1-Met2 &  -8.15 & 17:20:53.3454 & -35:46:57.753 & 3.04 (0.01)\\
331 & MM1-Met2 &  -8.15 & 17:20:53.3632 & -35:46:58.481 & 0.608 (0.008)\\
332 & MM1-Met2 &  -8.15 & 17:20:53.3744 & -35:46:58.853 & 0.987 (0.008)\\
333 & MM1-Met2 &  -8.15 & 17:20:53.3162 & -35:46:57.838 & 0.560 (0.008)\\
334 & UCHII-Met3 &  -8.00 & 17:20:53.4051 & -35:47:02.134 & 0.707 (0.013)\\
335 & UCHII-Met5 &  -8.00 & 17:20:53.4359 & -35:47:01.532 & 16.9 (0.1)\\
336 & MM1-Met1 &  -8.00 & 17:20:53.4230 & -35:46:57.027 & 15.6 (0.1)\\
337 & MM1-Met1 &  -8.00 & 17:20:53.4161 & -35:46:56.991 & 14.5 (0.1)\\
338 & UCHII-Met2 &  -8.00 & 17:20:53.4134 & -35:47:02.632 & 10.9 (0.1)\\
339 & UCHII-Met1 &  -8.00 & 17:20:53.4097 & -35:47:03.351 & 0.707 (0.013)\\
340 & UCHII-Met5 &  -8.00 & 17:20:53.4095 & -35:47:01.340 & 2.34 (0.01)\\
341 & UCHII-Met6 &  -8.00 & 17:20:53.4031 & -35:46:59.946 & 0.329 (0.013)\\
342 & MM1-Met2 &  -8.00 & 17:20:53.3439 & -35:46:57.768 & 1.61 (0.01)\\
343 & CM2-Met1 &  -8.00 & 17:20:53.3882 & -35:46:55.686 & 0.339 (0.013)\\
344 & MM1-Met2 &  -8.00 & 17:20:53.3706 & -35:46:58.581 & 0.782 (0.013)\\
345 & MM1-Met2 &  -8.00 & 17:20:53.2946 & -35:46:57.959 & 0.453 (0.013)\\
346 & MM2-Met1 &  -8.00 & 17:20:53.1882 & -35:46:58.868 & 0.766 (0.013)\\
347 & MM2-Met1 &  -8.00 & 17:20:53.1602 & -35:46:59.347 & 3.57 (0.01)\\
348 & MM2-Met1 &  -8.00 & 17:20:53.1544 & -35:46:59.335 & 2.34 (0.01)\\
349 & MM2-Met2 &  -8.00 & 17:20:53.1294 & -35:46:58.557 & 4.19 (0.01)\\
350 & MM1-Met1 &  -8.00 & 17:20:53.3958 & -35:46:57.191 & 0.629 (0.013)\\
351 & UCHII-Met5 &  -7.85 & 17:20:53.4089 & -35:47:01.383 & 1.50 (0.04)\\
352 & UCHII-Met5 &  -7.85 & 17:20:53.4362 & -35:47:01.527 & 11.7 (0.1)\\
353 & MM1-Met1 &  -7.85 & 17:20:53.4231 & -35:46:57.027 & 48.3 (0.1)\\
354 & UCHII-Met1 &  -7.85 & 17:20:53.4154 & -35:47:03.200 & 1.17 (0.04)\\
355 & UCHII-Met2 &  -7.85 & 17:20:53.4128 & -35:47:02.580 & 6.84 (0.04)\\
356 & MM1-Met1 &  -7.85 & 17:20:53.3928 & -35:46:57.292 & 0.792 (0.036)\\
357 & MM1-Met1 &  -7.85 & 17:20:53.4168 & -35:46:56.985 & 42.8 (0.1)\\
358 & MM1-Met2 &  -7.85 & 17:20:53.3666 & -35:46:58.502 & 0.492 (0.036)\\
359 & MM1-Met2 &  -7.85 & 17:20:53.3429 & -35:46:57.788 & 0.340 (0.036)\\
360 & MM1-Met2 &  -7.85 & 17:20:53.2924 & -35:46:58.018 & 0.334 (0.036)\\
361 & MM2-Met1 &  -7.85 & 17:20:53.1875 & -35:46:58.879 & 0.741 (0.036)\\
362 & CM2-Met1 &  -7.85 & 17:20:53.3889 & -35:46:55.685 & 1.18 (0.04)\\
363 & MM2-Met1 &  -7.85 & 17:20:53.1568 & -35:46:59.340 & 3.86 (0.04)\\
364 & MM2-Met2 &  -7.85 & 17:20:53.1294 & -35:46:58.545 & 5.59 (0.04)\\
365 & UCHII-Met5 &  -7.70 & 17:20:53.4356 & -35:47:01.504 & 2.64 (0.09)\\
366 & MM1-Met1 &  -7.70 & 17:20:53.4215 & -35:46:57.027 & 115 (1)\\
367 & MM1-Met1 &  -7.70 & 17:20:53.4172 & -35:46:56.971 & 117 (1)\\
368 & UCHII-Met1 &  -7.70 & 17:20:53.4163 & -35:47:03.273 & 2.16 (0.09)\\
369 & UCHII-Met5 &  -7.70 & 17:20:53.4135 & -35:47:01.347 & 2.38 (0.09)\\
370 & CM2-Met1 &  -7.70 & 17:20:53.3816 & -35:46:55.646 & 3.10 (0.09)\\
371 & MM1-Met1 &  -7.70 & 17:20:53.3885 & -35:46:57.298 & 1.47 (0.09)\\
372 & MM2-Met1 &  -7.70 & 17:20:53.1529 & -35:46:59.347 & 1.25 (0.09)\\
373 & MM2-Met2 &  -7.70 & 17:20:53.1304 & -35:46:58.526 & 3.15 (0.09)\\
374 & UCHII-Met2 &  -7.70 & 17:20:53.4114 & -35:47:02.463 & 3.64 (0.09)\\
375 & MM1-Met1 &  -7.55 & 17:20:53.4178 & -35:46:56.970 & 343 (1)\\
376 & MM1-Met1 &  -7.55 & 17:20:53.4206 & -35:46:57.030 & 215 (1)\\
377 & UCHII-Met5 &  -7.55 & 17:20:53.4161 & -35:47:01.326 & 8.13 (0.16)\\
378 & UCHII-Met1 &  -7.55 & 17:20:53.4178 & -35:47:03.369 & 7.71 (0.16)\\
379 & MM1-Met1 &  -7.55 & 17:20:53.3987 & -35:46:57.350 & 2.26 (0.16)\\
380 & CM2-Met1 &  -7.55 & 17:20:53.3800 & -35:46:55.662 & 5.03 (0.16)\\
381 & UCHII-Met2 &  -7.55 & 17:20:53.4121 & -35:47:02.436 & 3.98 (0.16)\\
382 & CM2-Met1 &  -7.40 & 17:20:53.3788 & -35:46:55.731 & 3.68 (0.20)\\
383 & MM1-Met1 &  -7.40 & 17:20:53.3987 & -35:46:57.275 & 3.58 (0.20)\\
384 & UCHII-Met2 &  -7.40 & 17:20:53.4113 & -35:47:02.421 & 3.37 (0.20)\\
385 & UCHII-Met5 &  -7.40 & 17:20:53.4161 & -35:47:01.317 & 14.8 (0.2)\\
386 & MM1-Met1 &  -7.40 & 17:20:53.4167 & -35:46:56.955 & 271 (1)\\
387 & UCHII-Met1 &  -7.40 & 17:20:53.4174 & -35:47:03.379 & 34.6 (0.2)\\
388 & MM1-Met1 &  -7.40 & 17:20:53.4198 & -35:46:57.011 & 533 (1)\\
389 & UCHII-Met1 &  -7.40 & 17:20:53.4775 & -35:47:03.778 & 1.56 (0.20)\\
390 & UCHII-Met1 &  -7.25 & 17:20:53.4765 & -35:47:03.706 & 4.95 (0.17)\\
391 & UCHII-Met1 &  -7.25 & 17:20:53.4248 & -35:47:03.409 & 10.7 (0.2)\\
392 & MM1-Met1 &  -7.25 & 17:20:53.4199 & -35:46:57.006 & 545 (1)\\
393 & UCHII-Met1 &  -7.25 & 17:20:53.4168 & -35:47:03.376 & 30.0 (0.2)\\
394 & MM1-Met2 &  -7.25 & 17:20:53.3589 & -35:46:58.525 & 2.33 (0.17)\\
395 & MM1-Met1 &  -7.25 & 17:20:53.4139 & -35:46:56.945 & 159 (1)\\
396 & UCHII-Met2 &  -7.25 & 17:20:53.4111 & -35:47:02.363 & 2.16 (0.17)\\
397 & MM1-Met1 &  -7.25 & 17:20:53.4029 & -35:46:57.124 & 9.22 (0.17)\\
398 & UCHII-Met5 &  -7.25 & 17:20:53.4165 & -35:47:01.318 & 11.6 (0.2)\\
399 & UCHII-Met1 &  -7.10 & 17:20:53.4176 & -35:47:03.379 & 15.5 (0.1)\\
400 & UCHII-Met1 &  -7.10 & 17:20:53.4765 & -35:47:03.709 & 2.52 (0.13)\\
401 & MM1-Met1 &  -7.10 & 17:20:53.4217 & -35:46:57.025 & 237 (1)\\
402 & UCHII-Met5 &  -7.10 & 17:20:53.4166 & -35:47:01.317 & 7.28 (0.13)\\
403 & UCHII-Met1 &  -7.10 & 17:20:53.4256 & -35:47:03.401 & 22.8 (0.1)\\
404 & UCHII-Met2 &  -7.10 & 17:20:53.4103 & -35:47:02.393 & 1.45 (0.13)\\
405 & MM1-Met1 &  -7.10 & 17:20:53.4080 & -35:46:56.977 & 66.4 (0.1)\\
406 & MM1-Met1 &  -7.10 & 17:20:53.4157 & -35:46:56.963 & 203 (1)\\
407 & MM1-Met2 &  -7.10 & 17:20:53.3582 & -35:46:58.506 & 2.18 (0.13)\\
408 & UCHII-Met1 &  -6.95 & 17:20:53.4795 & -35:47:03.697 & 1.65 (0.10)\\
409 & UCHII-Met1 &  -6.95 & 17:20:53.4475 & -35:47:03.673 & 1.52 (0.10)\\
410 & UCHII-Met1 &  -6.95 & 17:20:53.4270 & -35:47:03.415 & 36.9 (0.1)\\
411 & MM1-Met1 &  -6.95 & 17:20:53.4237 & -35:46:57.040 & 139 (1)\\
412 & UCHII-Met1 &  -6.95 & 17:20:53.4209 & -35:47:03.362 & 22.0 (0.1)\\
413 & UCHII-Met5 &  -6.95 & 17:20:53.4166 & -35:47:01.296 & 4.51 (0.10)\\
414 & UCHII-Met2 &  -6.95 & 17:20:53.4085 & -35:47:02.250 & 0.800 (0.101)\\
415 & MM1-Met1 &  -6.95 & 17:20:53.4083 & -35:46:56.964 & 87.2 (0.1)\\
416 & MM1-Met2 &  -6.95 & 17:20:53.3580 & -35:46:58.490 & 1.40 (0.10)\\
417 & MM1-Met1 &  -6.95 & 17:20:53.4173 & -35:46:56.977 & 128 (1)\\
418 & UCHII-Met1 &  -6.80 & 17:20:53.4220 & -35:47:03.355 & 28.5 (0.1)\\
419 & UCHII-Met1 &  -6.80 & 17:20:53.4804 & -35:47:03.705 & 2.72 (0.09)\\
420 & UCHII-Met1 &  -6.80 & 17:20:53.4395 & -35:47:03.587 & 19.5 (0.1)\\
421 & UCHII-Met1 &  -6.80 & 17:20:53.4281 & -35:47:03.432 & 48.0 (0.1)\\
422 & MM1-Met1 &  -6.80 & 17:20:53.4227 & -35:46:57.026 & 216 (1)\\
423 & UCHII-Met5 &  -6.80 & 17:20:53.4161 & -35:47:01.293 & 1.90 (0.09)\\
424 & CM2-Met2 &  -6.80 & 17:20:53.4102 & -35:46:55.800 & 2.73 (0.09)\\
425 & MM1-Met1 &  -6.80 & 17:20:53.4067 & -35:46:56.932 & 84.7 (0.1)\\
426 & UCHII-Met2 &  -6.80 & 17:20:53.4059 & -35:47:02.205 & 2.39 (0.09)\\
427 & MM1-Met1 &  -6.80 & 17:20:53.3904 & -35:46:56.895 & 5.23 (0.09)\\
428 & MM1-Met2 &  -6.80 & 17:20:53.3588 & -35:46:58.381 & 0.694 (0.089)\\
429 & MM2-Met2 &  -6.80 & 17:20:53.1505 & -35:46:58.105 & 2.33 (0.09)\\
430 & UCHII-Met1 &  -6.65 & 17:20:53.4771 & -35:47:03.684 & 0.514 (0.061)\\
431 & MM1-Met1 &  -6.65 & 17:20:53.4398 & -35:46:56.400 & 1.21 (0.06)\\
432 & UCHII-Met1 &  -6.65 & 17:20:53.4372 & -35:47:03.558 & 93.0 (0.1)\\
433 & UCHII-Met1 &  -6.65 & 17:20:53.4259 & -35:47:03.405 & 42.8 (0.1)\\
434 & MM1-Met1 &  -6.65 & 17:20:53.4229 & -35:46:57.032 & 145 (1)\\
435 & CM2-Met2 &  -6.65 & 17:20:53.4103 & -35:46:55.850 & 4.98 (0.06)\\
436 & UCHII-Met2 &  -6.65 & 17:20:53.4063 & -35:47:02.205 & 5.60 (0.06)\\
437 & MM1-Met1 &  -6.65 & 17:20:53.4031 & -35:46:56.906 & 177 (1)\\
438 & MM1-Met1 &  -6.65 & 17:20:53.3822 & -35:46:57.150 & 2.66 (0.06)\\
439 & MM2-Met2 &  -6.65 & 17:20:53.1534 & -35:46:58.116 & 2.87 (0.06)\\
440 & MM1-Met1 &  -6.50 & 17:20:53.4381 & -35:46:56.421 & 1.41 (0.05)\\
441 & MM1-Met1 &  -6.50 & 17:20:53.4452 & -35:46:58.010 & 1.03 (0.05)\\
442 & UCHII-Met1 &  -6.50 & 17:20:53.4273 & -35:47:03.426 & 29.3 (0.1)\\
443 & MM1-Met1 &  -6.50 & 17:20:53.4230 & -35:46:57.037 & 72.2 (0.1)\\
444 & UCHII-Met1 &  -6.50 & 17:20:53.4368 & -35:47:03.556 & 79.2 (0.1)\\
445 & UCHII-Met2 &  -6.50 & 17:20:53.4059 & -35:47:02.220 & 4.03 (0.05)\\
446 & MM1-Met1 &  -6.50 & 17:20:53.4022 & -35:46:56.908 & 295 (1)\\
447 & MM1-Met1 &  -6.50 & 17:20:53.3835 & -35:46:57.151 & 2.43 (0.05)\\
448 & MM2-Met2 &  -6.50 & 17:20:53.1562 & -35:46:58.127 & 1.99 (0.05)\\
449 & CM2-Met2 &  -6.50 & 17:20:53.4111 & -35:46:55.842 & 4.30 (0.05)\\
450 & MM1-MetC &  -6.35 & 17:20:53.4435 & -35:46:58.296 & 1.34 (0.04)\\
451 & MM1-Met1 &  -6.35 & 17:20:53.4375 & -35:46:56.365 & 1.03 (0.04)\\
452 & UCHII-Met1 &  -6.35 & 17:20:53.4343 & -35:47:03.528 & 20.2 (0.1)\\
453 & UCHII-Met1 &  -6.35 & 17:20:53.4236 & -35:47:03.401 & 8.28 (0.04)\\
454 & MM1-Met1 &  -6.35 & 17:20:53.4230 & -35:46:57.044 & 27.1 (0.1)\\
455 & CM2-Met2 &  -6.35 & 17:20:53.4125 & -35:46:55.793 & 2.25 (0.04)\\
456 & UCHII-Met2 &  -6.35 & 17:20:53.4072 & -35:47:02.183 & 0.516 (0.039)\\
457 & MM1-Met1 &  -6.35 & 17:20:53.4016 & -35:46:56.912 & 235 (1)\\
458 & MM1-Met1 &  -6.35 & 17:20:53.3821 & -35:46:57.222 & 1.33 (0.04)\\
459 & MM2-Met2 &  -6.35 & 17:20:53.1570 & -35:46:58.160 & 1.10 (0.04)\\
460 & MM1-MetC &  -6.20 & 17:20:53.4453 & -35:46:58.268 & 1.51 (0.02)\\
461 & MM1-Met1 &  -6.20 & 17:20:53.4417 & -35:46:56.400 & 0.756 (0.023)\\
462 & UCHII-Met1 &  -6.20 & 17:20:53.4521 & -35:47:03.671 & 0.164 (0.023)\\
463 & MM1-Met1 &  -6.20 & 17:20:53.4244 & -35:46:57.043 & 8.20 (0.02)\\
464 & UCHII-Met1 &  -6.20 & 17:20:53.4189 & -35:47:03.375 & 1.86 (0.02)\\
465 & UCHII-Met1 &  -6.20 & 17:20:53.4328 & -35:47:03.522 & 1.51 (0.02)\\
466 & MM1-Met1 &  -6.20 & 17:20:53.4071 & -35:46:57.012 & 6.33 (0.02)\\
467 & MM1-Met1 &  -6.20 & 17:20:53.4004 & -35:46:56.912 & 68.2 (0.1)\\
468 & MM1-Met1 &  -6.20 & 17:20:53.3786 & -35:46:57.329 & 0.407 (0.023)\\
469 & MM2-Met2 &  -6.20 & 17:20:53.1585 & -35:46:58.105 & 0.341 (0.023)\\
470 & CM2-Met2 &  -6.20 & 17:20:53.4148 & -35:46:55.836 & 1.34 (0.02)\\
471 & UCHII-Met1 &  -6.05 & 17:20:53.4533 & -35:47:03.643 & 0.320 (0.006)\\
472 & MM1-MetC &  -6.05 & 17:20:53.4451 & -35:46:58.290 & 1.27 (0.01)\\
473 & MM1-Met1 &  -6.05 & 17:20:53.4419 & -35:46:56.500 & 0.560 (0.006)\\
474 & UCHII-Met1 &  -6.05 & 17:20:53.4349 & -35:47:03.531 & 0.197 (0.006)\\
475 & MM1-Met1 &  -6.05 & 17:20:53.4262 & -35:46:57.068 & 2.96 (0.01)\\
476 & UCHII-Met1 &  -6.05 & 17:20:53.4190 & -35:47:03.372 & 0.295 (0.006)\\
477 & CM2-Met2 &  -6.05 & 17:20:53.4177 & -35:46:55.861 & 0.594 (0.006)\\
478 & MM1-Met1 &  -6.05 & 17:20:53.4002 & -35:46:56.925 & 9.86 (0.01)\\
479 & MM1-Met1 &  -6.05 & 17:20:53.3997 & -35:46:57.570 & 0.282 (0.006)\\
480 & MM1-Met2 &  -6.05 & 17:20:53.3744 & -35:46:57.375 & 0.256 (0.006)\\
481 & MM1-Met2 &  -6.05 & 17:20:53.3544 & -35:46:57.714 & 0.406 (0.006)\\
482 & MM1-Met2 &  -6.05 & 17:20:53.3222 & -35:46:57.214 & 0.216 (0.006)\\
483 & MM2-Met2 &  -6.05 & 17:20:53.1544 & -35:46:58.176 & 0.0944 (0.0062)\\
484 & MM1-Met1 &  -6.05 & 17:20:53.4138 & -35:46:56.974 & 1.01 (0.01)\\
485 & MM1-Met1 &  -5.90 & 17:20:53.4368 & -35:46:56.942 & 0.769 (0.003)\\
486 & MM1-Met1 &  -5.90 & 17:20:53.4569 & -35:46:56.756 & 0.224 (0.003)\\
487 & UCHII-Met1 &  -5.90 & 17:20:53.4559 & -35:47:03.691 & 0.588 (0.003)\\
488 & MM1-MetC &  -5.90 & 17:20:53.4456 & -35:46:58.284 & 0.849 (0.003)\\
489 & MM1-Met1 &  -5.90 & 17:20:53.4398 & -35:46:56.185 & 0.227 (0.003)\\
490 & UCHII-Met1 &  -5.90 & 17:20:53.4299 & -35:47:03.459 & 0.0771 (0.0031)\\
491 & MM1-Met2 &  -5.90 & 17:20:53.3217 & -35:46:57.296 & 0.240 (0.003)\\
492 & CM2-Met2 &  -5.90 & 17:20:53.4203 & -35:46:55.882 & 0.288 (0.003)\\
493 & MM1-Met2 &  -5.90 & 17:20:53.3535 & -35:46:57.711 & 0.487 (0.003)\\
494 & MM1-Met2 &  -5.90 & 17:20:53.3725 & -35:46:57.417 & 0.201 (0.003)\\
495 & MM1-Met1 &  -5.90 & 17:20:53.4238 & -35:46:57.061 & 1.32 (0.01)\\
496 & MM1-Met1 &  -5.90 & 17:20:53.4045 & -35:46:56.933 & 0.675 (0.003)\\
497 & MM1-Met1 &  -5.90 & 17:20:53.3983 & -35:46:57.460 & 0.559 (0.003)\\
498 & UCHII-Met1 &  -5.75 & 17:20:53.4562 & -35:47:03.699 & 0.467 (0.003)\\
499 & MM1-MetC &  -5.75 & 17:20:53.4438 & -35:46:58.353 & 0.397 (0.003)\\
500 & MM1-Met1 &  -5.75 & 17:20:53.4403 & -35:46:56.076 & 0.198 (0.003)\\
501 & MM1-Met1 &  -5.75 & 17:20:53.4381 & -35:46:56.897 & 1.55 (0.01)\\
502 & UCHII-Met1 &  -5.75 & 17:20:53.4284 & -35:47:03.404 & 0.0372 (0.0029)\\
503 & CM2-Met2 &  -5.75 & 17:20:53.4248 & -35:46:55.925 & 0.345 (0.003)\\
504 & MM1-Met1 &  -5.75 & 17:20:53.4573 & -35:46:56.701 & 0.287 (0.003)\\
505 & MM1-Met1 &  -5.75 & 17:20:53.4066 & -35:46:56.929 & 0.422 (0.003)\\
506 & MM1-Met1 &  -5.75 & 17:20:53.4240 & -35:46:57.056 & 0.658 (0.003)\\
507 & MM1-Met2 &  -5.75 & 17:20:53.3103 & -35:46:57.687 & 0.135 (0.003)\\
508 & MM1-Met2 &  -5.75 & 17:20:53.3227 & -35:46:57.331 & 0.252 (0.003)\\
509 & MM1-Met1 &  -5.75 & 17:20:53.4545 & -35:46:57.989 & 0.230 (0.003)\\
510 & MM1-Met2 &  -5.75 & 17:20:53.3722 & -35:46:57.412 & 0.151 (0.003)\\
511 & MM1-Met1 &  -5.75 & 17:20:53.3983 & -35:46:57.455 & 0.421 (0.003)\\
512 & MM1-Met2 &  -5.75 & 17:20:53.3532 & -35:46:57.676 & 0.460 (0.003)\\
513 & CM2-Met2 &  -5.60 & 17:20:53.4278 & -35:46:55.979 & 0.715 (0.003)\\
514 & MM1-Met1 &  -5.60 & 17:20:53.4580 & -35:46:56.955 & 0.230 (0.003)\\
515 & UCHII-Met1 &  -5.60 & 17:20:53.4555 & -35:47:03.705 & 0.0683 (0.0029)\\
516 & MM1-Met1 &  -5.60 & 17:20:53.4551 & -35:46:57.994 & 0.221 (0.003)\\
517 & MM1-Met1 &  -5.60 & 17:20:53.4528 & -35:46:56.337 & 0.258 (0.003)\\
518 & MM1-MetC &  -5.60 & 17:20:53.4417 & -35:46:58.395 & 0.192 (0.003)\\
519 & MM1-Met1 &  -5.60 & 17:20:53.4381 & -35:46:56.887 & 3.63 (0.01)\\
520 & MM1-Met1 &  -5.60 & 17:20:53.4028 & -35:46:57.079 & 0.330 (0.003)\\
521 & MM1-Met1 &  -5.60 & 17:20:53.4209 & -35:46:57.021 & 0.432 (0.003)\\
522 & MM1-Met1 &  -5.60 & 17:20:53.3775 & -35:46:57.408 & 0.117 (0.003)\\
523 & MM1-Met2 &  -5.60 & 17:20:53.3532 & -35:46:57.562 & 0.398 (0.003)\\
524 & MM1-Met2 &  -5.60 & 17:20:53.3210 & -35:46:57.490 & 0.340 (0.003)\\
525 & MM1-Met2 &  -5.60 & 17:20:53.3044 & -35:46:57.654 & 0.174 (0.003)\\
526 & UCHII-Met1 &  -5.60 & 17:20:53.4291 & -35:47:03.308 & 0.0282 (0.0029)\\
527 & MM1-Met1 &  -5.45 & 17:20:53.4564 & -35:46:57.831 & 0.199 (0.004)\\
528 & MM1-Met1 &  -5.45 & 17:20:53.4530 & -35:46:56.648 & 0.459 (0.004)\\
529 & MM1-Met1 &  -5.45 & 17:20:53.4380 & -35:46:56.880 & 9.98 (0.01)\\
530 & MM1-Met1 &  -5.45 & 17:20:53.4289 & -35:46:56.006 & 0.996 (0.004)\\
531 & MM1-Met2 &  -5.45 & 17:20:53.3527 & -35:46:57.464 & 0.352 (0.004)\\
532 & MM1-Met2 &  -5.45 & 17:20:53.3201 & -35:46:57.554 & 0.367 (0.004)\\
533 & MM1-Met2 &  -5.45 & 17:20:53.3034 & -35:46:57.637 & 0.231 (0.004)\\
534 & MM1-Met1 &  -5.45 & 17:20:53.4142 & -35:46:57.038 & 0.304 (0.004)\\
535 & MM1-Met1 &  -5.30 & 17:20:53.4558 & -35:46:56.790 & 0.315 (0.009)\\
536 & MM1-Met1 &  -5.30 & 17:20:53.4381 & -35:46:56.873 & 35.3 (0.1)\\
537 & CM2-Met2 &  -5.30 & 17:20:53.4251 & -35:46:55.946 & 0.628 (0.009)\\
538 & MM1-Met1 &  -5.30 & 17:20:53.4368 & -35:46:56.176 & 0.638 (0.009)\\
539 & MM1-Met2 &  -5.30 & 17:20:53.3200 & -35:46:57.567 & 0.351 (0.009)\\
540 & MM1-Met2 &  -5.30 & 17:20:53.3041 & -35:46:57.655 & 0.250 (0.009)\\
541 & MM1-Met2 &  -5.30 & 17:20:53.3499 & -35:46:57.428 & 0.335 (0.009)\\
542 & MM1-Met1 &  -5.15 & 17:20:53.4381 & -35:46:56.870 & 83.1 (0.1)\\
543 & MM1-Met2 &  -5.15 & 17:20:53.3011 & -35:46:57.654 & 0.251 (0.019)\\
544 & MM1-Met2 &  -5.15 & 17:20:53.3188 & -35:46:57.545 & 0.420 (0.019)\\
545 & MM1-Met2 &  -5.15 & 17:20:53.3470 & -35:46:57.417 & 0.362 (0.019)\\
546 & MM1-Met1 &  -5.15 & 17:20:53.4362 & -35:46:56.164 & 0.969 (0.019)\\
547 & MM1-Met1 &  -5.00 & 17:20:53.4381 & -35:46:56.871 & 80.0 (0.1)\\
548 & MM1-Met1 &  -5.00 & 17:20:53.4389 & -35:46:56.329 & 1.33 (0.02)\\
549 & MM1-Met2 &  -5.00 & 17:20:53.3153 & -35:46:57.569 & 0.448 (0.018)\\
550 & MM1-Met2 &  -5.00 & 17:20:53.3440 & -35:46:57.415 & 0.402 (0.018)\\
551 & MM1-Met2 &  -4.85 & 17:20:53.3125 & -35:46:57.585 & 0.374 (0.009)\\
552 & MM1-Met2 &  -4.85 & 17:20:53.3321 & -35:46:57.540 & 0.407 (0.009)\\
553 & MM1-Met2 &  -4.85 & 17:20:53.3484 & -35:46:57.439 & 0.357 (0.009)\\
554 & MM1-Met1 &  -4.85 & 17:20:53.4343 & -35:46:56.939 & 2.40 (0.01)\\
555 & MM1-Met1 &  -4.85 & 17:20:53.4384 & -35:46:56.866 & 23.7 (0.1)\\
556 & MM1-Met1 &  -4.85 & 17:20:53.4399 & -35:46:56.329 & 1.36 (0.01)\\
557 & MM1-Met1 &  -4.70 & 17:20:53.4525 & -35:46:57.440 & 0.102 (0.004)\\
558 & MM1-Met1 &  -4.70 & 17:20:53.4407 & -35:46:56.365 & 1.09 (0.01)\\
559 & MM1-Met1 &  -4.70 & 17:20:53.4378 & -35:46:56.880 & 2.52 (0.01)\\
560 & MM1-Met1 &  -4.70 & 17:20:53.4284 & -35:46:56.978 & 0.357 (0.004)\\
561 & MM1-Met2 &  -4.70 & 17:20:53.3369 & -35:46:57.630 & 0.764 (0.004)\\
562 & MM1-Met2 &  -4.70 & 17:20:53.3417 & -35:46:57.271 & 0.165 (0.004)\\
563 & MM1-Met2 &  -4.70 & 17:20:53.3229 & -35:46:57.583 & 0.349 (0.004)\\
564 & MM1-Met2 &  -4.70 & 17:20:53.3078 & -35:46:57.555 & 0.225 (0.004)\\
565 & MM1-Met2 &  -4.70 & 17:20:53.3512 & -35:46:57.481 & 0.297 (0.004)\\
566 & MM1-Met3 &  -4.55 & 17:20:53.5112 & -35:46:57.875 & 0.0251 (0.0022)\\
567 & MM1-Met1 &  -4.55 & 17:20:53.4525 & -35:46:57.439 & 0.0578 (0.0022)\\
568 & MM1-Met1 &  -4.55 & 17:20:53.4411 & -35:46:56.380 & 0.553 (0.002)\\
569 & MM1-Met1 &  -4.55 & 17:20:53.4348 & -35:46:56.929 & 0.788 (0.002)\\
570 & MM1-Met1 &  -4.55 & 17:20:53.4266 & -35:46:56.971 & 0.199 (0.002)\\
571 & MM1-Met2 &  -4.55 & 17:20:53.3418 & -35:46:57.337 & 0.315 (0.002)\\
572 & MM1-Met2 &  -4.55 & 17:20:53.3365 & -35:46:57.640 & 1.32 (0.01)\\
573 & MM1-Met2 &  -4.55 & 17:20:53.3084 & -35:46:57.543 & 0.217 (0.002)\\
574 & MM1-Met2 &  -4.55 & 17:20:53.3518 & -35:46:57.471 & 0.563 (0.002)\\
575 & MM1-Met2 &  -4.55 & 17:20:53.3238 & -35:46:57.597 & 0.512 (0.002)\\
576 & MM1-Met2 &  -4.40 & 17:20:53.3093 & -35:46:57.551 & 0.192 (0.002)\\
577 & MM1-Met2 &  -4.40 & 17:20:53.3244 & -35:46:57.606 & 0.615 (0.002)\\
578 & MM1-Met2 &  -4.40 & 17:20:53.3361 & -35:46:57.639 & 1.32 (0.01)\\
579 & MM1-Met2 &  -4.40 & 17:20:53.3435 & -35:46:57.361 & 0.465 (0.002)\\
580 & MM1-Met1 &  -4.40 & 17:20:53.4208 & -35:46:57.011 & 0.0535 (0.0021)\\
581 & MM1-Met1 &  -4.40 & 17:20:53.4329 & -35:46:56.918 & 1.12 (0.01)\\
582 & MM1-Met1 &  -4.40 & 17:20:53.4414 & -35:46:56.382 & 0.198 (0.002)\\
583 & MM1-Met1 &  -4.40 & 17:20:53.4485 & -35:46:57.492 & 0.0417 (0.0021)\\
584 & MM1-Met3 &  -4.40 & 17:20:53.5112 & -35:46:57.907 & 0.0264 (0.0021)\\
585 & MM1-Met2 &  -4.40 & 17:20:53.3526 & -35:46:57.464 & 0.930 (0.002)\\
586 & MM1-Met3 &  -4.25 & 17:20:53.5077 & -35:46:57.905 & 0.0342 (0.0022)\\
587 & MM1-Met2 &  -4.25 & 17:20:53.3543 & -35:46:57.474 & 0.770 (0.002)\\
588 & MM1-Met1 &  -4.25 & 17:20:53.4398 & -35:46:56.498 & 0.0886 (0.0022)\\
589 & MM1-Met1 &  -4.25 & 17:20:53.4324 & -35:46:56.918 & 1.43 (0.01)\\
590 & MM1-Met2 &  -4.25 & 17:20:53.3476 & -35:46:57.414 & 0.748 (0.002)\\
591 & MM1-Met2 &  -4.25 & 17:20:53.3225 & -35:46:57.610 & 0.484 (0.002)\\
592 & MM1-Met2 &  -4.25 & 17:20:53.3072 & -35:46:57.522 & 0.0958 (0.0022)\\
593 & MM1-Met2 &  -4.25 & 17:20:53.3347 & -35:46:57.631 & 0.951 (0.002)\\
594 & MM1-Met3 &  -4.10 & 17:20:53.5050 & -35:46:57.914 & 0.0473 (0.0021)\\
595 & MM1-Met1 &  -4.10 & 17:20:53.4322 & -35:46:56.914 & 1.22 (0.01)\\
596 & MM1-Met2 &  -4.10 & 17:20:53.3536 & -35:46:57.450 & 0.771 (0.002)\\
597 & MM1-Met1 &  -4.10 & 17:20:53.4398 & -35:46:56.581 & 0.0502 (0.0021)\\
598 & MM1-Met2 &  -4.10 & 17:20:53.3311 & -35:46:57.629 & 0.641 (0.002)\\
599 & MM1-Met2 &  -4.10 & 17:20:53.3167 & -35:46:57.583 & 0.203 (0.002)\\
600 & MM1-Met2 &  -4.10 & 17:20:53.3437 & -35:46:57.510 & 0.438 (0.002)\\
601 & MM1-Met2 &  -3.95 & 17:20:53.3228 & -35:46:57.610 & 0.228 (0.002)\\
602 & MM1-Met2 &  -3.95 & 17:20:53.3365 & -35:46:57.578 & 0.626 (0.002)\\
603 & MM1-Met2 &  -3.95 & 17:20:53.3528 & -35:46:57.468 & 0.500 (0.002)\\
604 & MM1-Met1 &  -3.95 & 17:20:53.4322 & -35:46:56.917 & 0.570 (0.002)\\
605 & MM1-Met3 &  -3.95 & 17:20:53.5029 & -35:46:57.889 & 0.0697 (0.0020)\\
606 & MM1-Met3 &  -3.80 & 17:20:53.4996 & -35:46:57.899 & 0.0830 (0.0021)\\
607 & MM1-Met2 &  -3.80 & 17:20:53.3535 & -35:46:57.480 & 0.256 (0.002)\\
608 & MM1-Met1 &  -3.80 & 17:20:53.4316 & -35:46:56.940 & 0.224 (0.002)\\
609 & MM1-Met2 &  -3.80 & 17:20:53.3248 & -35:46:57.567 & 0.150 (0.002)\\
610 & MM1-Met2 &  -3.80 & 17:20:53.3372 & -35:46:57.565 & 0.849 (0.002)\\
611 & MM1-Met2 &  -3.65 & 17:20:53.3295 & -35:46:57.524 & 0.190 (0.002)\\
612 & MM1-Met2 &  -3.65 & 17:20:53.3381 & -35:46:57.563 & 1.27 (0.01)\\
613 & MM1-Met2 &  -3.65 & 17:20:53.3541 & -35:46:57.500 & 0.135 (0.002)\\
614 & MM1-Met1 &  -3.65 & 17:20:53.4306 & -35:46:56.979 & 0.142 (0.002)\\
615 & MM1-Met3 &  -3.65 & 17:20:53.4967 & -35:46:57.897 & 0.104 (0.002)\\
616 & MM1-Met3 &  -3.50 & 17:20:53.4946 & -35:46:57.898 & 0.111 (0.002)\\
617 & MM1-Met1 &  -3.50 & 17:20:53.4299 & -35:46:57.002 & 0.115 (0.002)\\
618 & MM1-Met2 &  -3.50 & 17:20:53.3463 & -35:46:57.585 & 0.250 (0.002)\\
619 & MM1-Met2 &  -3.50 & 17:20:53.3372 & -35:46:57.552 & 1.39 (0.01)\\
620 & MM1-Met2 &  -3.35 & 17:20:53.3052 & -35:46:57.311 & 0.0182 (0.0019)\\
621 & MM1-Met2 &  -3.35 & 17:20:53.3375 & -35:46:57.552 & 0.736 (0.002)\\
622 & MM1-Met2 &  -3.35 & 17:20:53.3442 & -35:46:57.574 & 0.274 (0.002)\\
623 & MM1-Met1 &  -3.35 & 17:20:53.4290 & -35:46:57.011 & 0.0936 (0.0019)\\
624 & MM1-Met3 &  -3.35 & 17:20:53.4926 & -35:46:57.903 & 0.0838 (0.0019)\\
625 & MM1-Met3 &  -3.20 & 17:20:53.4915 & -35:46:57.860 & 0.0323 (0.0017)\\
626 & MM1-Met2 &  -3.20 & 17:20:53.3457 & -35:46:57.561 & 0.107 (0.002)\\
627 & MM1-Met1 &  -3.20 & 17:20:53.4280 & -35:46:57.028 & 0.0783 (0.0017)\\
628 & MM1-Met2 &  -3.20 & 17:20:53.3112 & -35:46:57.323 & 0.0234 (0.0017)\\
629 & MM1-Met2 &  -3.20 & 17:20:53.3387 & -35:46:57.565 & 0.234 (0.002)\\
630 & MM1-Met2 &  -3.05 & 17:20:53.3126 & -35:46:57.321 & 0.0262 (0.0016)\\
631 & MM1-Met2 &  -3.05 & 17:20:53.3423 & -35:46:57.563 & 0.0940 (0.0016)\\
632 & MM1-Met1 &  -3.05 & 17:20:53.4283 & -35:46:57.043 & 0.0760 (0.0016)\\
633 & MM1-Met2 &  -2.90 & 17:20:53.3149 & -35:46:57.252 & 0.0124 (0.0016)\\
634 & MM1-Met2 &  -2.90 & 17:20:53.3411 & -35:46:57.517 & 0.0307 (0.0016)\\
635 & MM1-Met1 &  -2.90 & 17:20:53.4282 & -35:46:57.054 & 0.0646 (0.0016)\\
636 & MM1-Met1 &  -2.75 & 17:20:53.4279 & -35:46:57.056 & 0.0524 (0.0016)\\
637 & MM1-Met2 &  -2.75 & 17:20:53.3377 & -35:46:57.474 & 0.0124 (0.0016)\\
638 & MM1-Met1 &  -2.60 & 17:20:53.4278 & -35:46:57.057 & 0.0513 (0.0015)\\
639 & MM2-Met2 &  -2.45 & 17:20:53.1256 & -35:46:58.328 & 0.0252 (0.0016)\\
640 & MM1-Met1 &  -2.45 & 17:20:53.4270 & -35:46:57.070 & 0.0475 (0.0016)\\
641 & MM2-Met2 &  -2.30 & 17:20:53.1246 & -35:46:58.367 & 0.0194 (0.0015)\\
642 & MM1-Met1 &  -2.30 & 17:20:53.4273 & -35:46:57.095 & 0.0477 (0.0015)\\
643 & MM1-Met1 &  -2.15 & 17:20:53.4272 & -35:46:57.084 & 0.0390 (0.0015)\\
644 & MM1-Met1 &  -2.00 & 17:20:53.4267 & -35:46:57.109 & 0.0329 (0.0015)\\
645 & MM1-Met1 &  -1.85 & 17:20:53.4263 & -35:46:57.157 & 0.0243 (0.0015)\\
646 & MM1-Met1 &  -1.70 & 17:20:53.4250 & -35:46:57.143 & 0.0171 (0.0015)\\
647 & MM1-Met1 &  -1.55 & 17:20:53.4225 & -35:46:57.011 & 0.0168 (0.0015)\\


==> oh_6030LLtable.tex <==
  1 & UCHII-OH4 & -11.00 & 17:20:53.3718 & -35:47:01.573 & 0.0241 (0.0025)\\
  2 & UCHII-OH4 & -10.85 & 17:20:53.3722 & -35:47:01.573 & 0.0903 (0.0022)\\
  3 & UCHII-OH6 & -10.85 & 17:20:53.3975 & -35:47:00.737 & 0.0294 (0.0022)\\
  4 & UCHII-OH4 & -10.70 & 17:20:53.3712 & -35:47:01.531 & 0.326 (0.002)\\
  5 & UCHII-OH6 & -10.70 & 17:20:53.3967 & -35:47:00.768 & 0.203 (0.002)\\
  6 & UCHII-OH4 & -10.55 & 17:20:53.3709 & -35:47:01.525 & 2.84 (0.01)\\
  7 & UCHII-OH6 & -10.55 & 17:20:53.3972 & -35:47:00.775 & 0.348 (0.004)\\
  8 & UCHII-OH4 & -10.40 & 17:20:53.3709 & -35:47:01.525 & 13.3 (0.1)\\
  9 & UCHII-OH6 & -10.40 & 17:20:53.3979 & -35:47:00.780 & 0.253 (0.007)\\
 10 & UCHII-OH4 & -10.25 & 17:20:53.3709 & -35:47:01.524 & 16.6 (0.1)\\
 11 & UCHII-OH6 & -10.25 & 17:20:53.3981 & -35:47:00.786 & 0.156 (0.010)\\
 12 & UCHII-OH6 & -10.10 & 17:20:53.3985 & -35:47:00.929 & 0.0608 (0.0043)\\
 13 & UCHII-OH4 & -10.10 & 17:20:53.3709 & -35:47:01.523 & 4.72 (0.01)\\
 14 & UCHII-OH4 &  -9.95 & 17:20:53.3712 & -35:47:01.514 & 0.0952 (0.0029)\\
 15 & UCHII-OH4 &  -9.80 & 17:20:53.3728 & -35:47:01.446 & 0.0170 (0.0025)\\
 16 & UCHII-OH2 &  -8.90 & 17:20:53.4081 & -35:47:02.783 & 0.0214 (0.0025)\\
 17 & UCHII-OH2 &  -8.75 & 17:20:53.4121 & -35:47:02.648 & 0.193 (0.003)\\
 18 & UCHII-OH2 &  -8.60 & 17:20:53.4125 & -35:47:02.645 & 0.428 (0.003)\\
 19 & UCHII-OH3 &  -8.60 & 17:20:53.4174 & -35:47:01.910 & 0.216 (0.003)\\
 20 & UCHII-OH2 &  -8.45 & 17:20:53.4129 & -35:47:02.653 & 0.558 (0.003)\\
 21 & UCHII-OH3 &  -8.45 & 17:20:53.4168 & -35:47:01.936 & 0.572 (0.003)\\
 22 & UCHII-OH5 &  -8.45 & 17:20:53.4220 & -35:47:01.458 & 0.140 (0.003)\\
 23 & UCHII-OH3 &  -8.30 & 17:20:53.4167 & -35:47:01.950 & 0.261 (0.003)\\
 24 & UCHII-OH5 &  -8.30 & 17:20:53.4216 & -35:47:01.428 & 0.226 (0.003)\\
 25 & UCHII-OH2 &  -8.30 & 17:20:53.4129 & -35:47:02.646 & 0.667 (0.003)\\
 26 & CM2-OH1-1 &  -8.15 & 17:20:53.3749 & -35:46:55.669 & 0.351 (0.003)\\
 27 & CM2-OH1-1 &  -8.15 & 17:20:53.3936 & -35:46:55.615 & 0.0748 (0.0025)\\
 28 & UCHII-OH2 &  -8.15 & 17:20:53.4127 & -35:47:02.645 & 0.233 (0.003)\\
 29 & UCHII-OH5 &  -8.15 & 17:20:53.4213 & -35:47:01.435 & 0.0503 (0.0025)\\
 30 & CM2-OH1-1 &  -8.00 & 17:20:53.3752 & -35:46:55.657 & 3.36 (0.01)\\
 31 & CM2-OH1-1 &  -8.00 & 17:20:53.3923 & -35:46:55.629 & 0.533 (0.003)\\
 32 & UCHII-OH2 &  -8.00 & 17:20:53.4149 & -35:47:02.666 & 0.177 (0.003)\\
 33 & CM2-OH1-1 &  -7.85 & 17:20:53.3754 & -35:46:55.654 & 6.70 (0.01)\\
 34 & CM2-OH1-1 &  -7.85 & 17:20:53.3919 & -35:46:55.615 & 1.32 (0.01)\\
 35 & UCHII-OH2 &  -7.85 & 17:20:53.4154 & -35:47:02.669 & 0.509 (0.003)\\
 36 & CM2-OH1-1 &  -7.70 & 17:20:53.3919 & -35:46:55.604 & 1.13 (0.01)\\
 37 & UCHII-OH2 &  -7.70 & 17:20:53.4154 & -35:47:02.667 & 0.311 (0.003)\\
 38 & CM2-OH1-1 &  -7.70 & 17:20:53.3766 & -35:46:55.636 & 4.24 (0.01)\\
 39 & CM2-OH1-1 &  -7.55 & 17:20:53.3794 & -35:46:55.598 & 2.87 (0.01)\\
 40 & CM2-OH1-1 &  -7.55 & 17:20:53.3919 & -35:46:55.592 & 0.205 (0.003)\\
 41 & UCHII-OH2 &  -7.55 & 17:20:53.4148 & -35:47:02.657 & 0.283 (0.003)\\
 42 & CM2-OH1-1 &  -7.40 & 17:20:53.3796 & -35:46:55.595 & 1.43 (0.01)\\
 43 & UCHII-OH2 &  -7.40 & 17:20:53.4149 & -35:47:02.653 & 1.08 (0.01)\\
 44 & CM2-OH1-1 &  -7.25 & 17:20:53.3799 & -35:46:55.589 & 0.0588 (0.0026)\\
 45 & UCHII-OH2 &  -7.25 & 17:20:53.4149 & -35:47:02.652 & 1.09 (0.01)\\
 46 & UCHII-OH2 &  -7.10 & 17:20:53.4147 & -35:47:02.657 & 0.195 (0.003)\\
 47 & UCHII-OH1 &  -6.65 & 17:20:53.4259 & -35:47:03.291 & 0.0573 (0.0027)\\
 48 & UCHII-OH1 &  -6.50 & 17:20:53.4256 & -35:47:03.304 & 0.0756 (0.0028)\\
 49 & UCHII-OH1 &  -6.35 & 17:20:53.4247 & -35:47:03.441 & 0.0121 (0.0026)\\


==> oh_6030RRtable.tex <==
  1 & UCHII-OH4 & -11.30 & 17:20:53.3687 & -35:47:01.536 & 0.0305 (0.0021)\\
  2 & UCHII-OH4 & -11.15 & 17:20:53.3704 & -35:47:01.533 & 0.113 (0.002)\\
  3 & UCHII-OH4 & -11.00 & 17:20:53.3709 & -35:47:01.527 & 0.973 (0.003)\\
  4 & UCHII-OH4 & -10.85 & 17:20:53.3709 & -35:47:01.525 & 6.56 (0.01)\\
  5 & UCHII-OH4 & -10.70 & 17:20:53.3709 & -35:47:01.524 & 13.0 (0.1)\\
  6 & UCHII-OH4 & -10.55 & 17:20:53.3709 & -35:47:01.523 & 6.78 (0.01)\\
  7 & UCHII-OH4 & -10.40 & 17:20:53.3708 & -35:47:01.527 & 0.639 (0.003)\\
  8 & UCHII-OH6 & -10.40 & 17:20:53.3964 & -35:47:00.796 & 0.128 (0.003)\\
  9 & UCHII-OH4 & -10.25 & 17:20:53.3702 & -35:47:01.547 & 0.0517 (0.0027)\\
 10 & UCHII-OH6 & -10.25 & 17:20:53.3967 & -35:47:00.776 & 0.332 (0.003)\\
 11 & UCHII-OH6 & -10.10 & 17:20:53.3962 & -35:47:00.783 & 0.324 (0.003)\\
 12 & UCHII-OH4 & -10.10 & 17:20:53.3685 & -35:47:01.528 & 0.0173 (0.0025)\\
 13 & UCHII-OH6 &  -9.95 & 17:20:53.3958 & -35:47:00.804 & 0.197 (0.002)\\
 14 & UCHII-OH6 &  -9.80 & 17:20:53.3948 & -35:47:00.834 & 0.0639 (0.0025)\\
 15 & UCHII-OH6 &  -9.65 & 17:20:53.3924 & -35:47:00.898 & 0.0137 (0.0025)\\
 16 & UCHII-OH2 &  -9.20 & 17:20:53.4103 & -35:47:02.669 & 0.0840 (0.0027)\\
 17 & UCHII-OH2 &  -9.05 & 17:20:53.4122 & -35:47:02.647 & 0.285 (0.003)\\
 18 & UCHII-OH2 &  -8.90 & 17:20:53.4127 & -35:47:02.660 & 0.384 (0.002)\\
 19 & UCHII-OH3 &  -8.90 & 17:20:53.4171 & -35:47:01.918 & 0.153 (0.002)\\
 20 & UCHII-OH2 &  -8.75 & 17:20:53.4130 & -35:47:02.650 & 0.598 (0.003)\\
 21 & UCHII-OH3 &  -8.75 & 17:20:53.4169 & -35:47:01.929 & 0.522 (0.003)\\
 22 & UCHII-OH2 &  -8.60 & 17:20:53.4128 & -35:47:02.639 & 0.393 (0.002)\\
 23 & UCHII-OH3 &  -8.60 & 17:20:53.4169 & -35:47:01.929 & 0.288 (0.002)\\
 24 & UCHII-OH3 &  -8.45 & 17:20:53.4186 & -35:47:01.845 & 0.00966 (0.00248)\\
 25 & UCHII-OH2 &  -8.45 & 17:20:53.4142 & -35:47:02.639 & 0.0896 (0.0025)\\
 26 & UCHII-OH2 &  -8.30 & 17:20:53.4156 & -35:47:02.664 & 0.352 (0.002)\\
 27 & UCHII-OH5 &  -8.30 & 17:20:53.4212 & -35:47:01.432 & 0.0199 (0.0024)\\
 28 & CM2-OH1-1 &  -8.15 & 17:20:53.3764 & -35:46:55.653 & 0.0364 (0.0024)\\
 29 & UCHII-OH2 &  -8.15 & 17:20:53.4154 & -35:47:02.665 & 0.516 (0.002)\\
 30 & UCHII-OH5 &  -8.15 & 17:20:53.4212 & -35:47:01.401 & 0.202 (0.002)\\
 31 & CM2-OH1-1 &  -8.00 & 17:20:53.3743 & -35:46:55.668 & 1.17 (0.01)\\
 32 & CM2-OH1-1 &  -8.00 & 17:20:53.3917 & -35:46:55.617 & 0.172 (0.003)\\
 33 & UCHII-OH2 &  -8.00 & 17:20:53.4149 & -35:47:02.663 & 0.312 (0.003)\\
 34 & UCHII-OH5 &  -8.00 & 17:20:53.4214 & -35:47:01.414 & 0.213 (0.003)\\
 35 & UCHII-OH2 &  -7.85 & 17:20:53.4148 & -35:47:02.653 & 0.945 (0.004)\\
 36 & CM2-OH1-1 &  -7.85 & 17:20:53.3894 & -35:46:55.606 & 0.818 (0.004)\\
 37 & CM2-OH1-1 &  -7.85 & 17:20:53.3747 & -35:46:55.661 & 6.55 (0.01)\\
 38 & CM2-OH1-1 &  -7.70 & 17:20:53.3753 & -35:46:55.653 & 8.50 (0.01)\\
 39 & CM2-OH1-1 &  -7.70 & 17:20:53.3889 & -35:46:55.596 & 1.35 (0.01)\\
 40 & UCHII-OH2 &  -7.70 & 17:20:53.4149 & -35:47:02.652 & 1.23 (0.01)\\
 41 & CM2-OH1-1 &  -7.55 & 17:20:53.3773 & -35:46:55.624 & 3.94 (0.01)\\
 42 & CM2-OH1-1 &  -7.55 & 17:20:53.3889 & -35:46:55.568 & 0.719 (0.004)\\
 43 & UCHII-OH2 &  -7.55 & 17:20:53.4150 & -35:47:02.652 & 0.328 (0.004)\\
 44 & CM2-OH1-1 &  -7.40 & 17:20:53.3797 & -35:46:55.591 & 1.66 (0.01)\\
 45 & CM2-OH1-1 &  -7.40 & 17:20:53.3928 & -35:46:55.693 & 0.0276 (0.0028)\\
 46 & UCHII-OH2 &  -7.40 & 17:20:53.4158 & -35:47:02.789 & 0.00679 (0.00283)\\
 47 & CM2-OH1-1 &  -7.25 & 17:20:53.3797 & -35:46:55.600 & 0.258 (0.003)\\
 48 & UCHII-OH1 &  -7.10 & 17:20:53.4266 & -35:47:03.360 & 0.0456 (0.0025)\\
 49 & UCHII-OH1 &  -6.95 & 17:20:53.4270 & -35:47:03.306 & 0.0709 (0.0026)\\
 50 & UCHII-OH1 &  -6.80 & 17:20:53.4286 & -35:47:03.329 & 0.00949 (0.00250)\\


==> oh_6035LLtable.tex <==
  1 & UCHII-OH4 & -12.05 & 17:20:53.3719 & -35:47:01.507 & 0.0231 (0.0022)\\
  2 & UCHII-OH4 & -11.90 & 17:20:53.3709 & -35:47:01.555 & 0.0281 (0.0024)\\
  3 & UCHII-OH4 & -11.75 & 17:20:53.3717 & -35:47:01.551 & 0.0376 (0.0024)\\
  4 & UCHII-OH4 & -11.60 & 17:20:53.3718 & -35:47:01.558 & 0.0672 (0.0021)\\
  5 & UCHII-OH4 & -11.45 & 17:20:53.3723 & -35:47:01.560 & 0.0972 (0.0025)\\
  6 & UCHII-OH4 & -11.15 & 17:20:53.3638 & -35:47:01.863 & 0.895 (0.009)\\
  7 & UCHII-OH4 & -11.15 & 17:20:53.3712 & -35:47:01.544 & 5.35 (0.01)\\
  8 & UCHII-OH4 & -11.00 & 17:20:53.3631 & -35:47:01.858 & 1.06 (0.01)\\
  9 & UCHII-OH4 & -11.00 & 17:20:53.3712 & -35:47:01.543 & 30.0 (0.1)\\
 10 & UCHII-OH4 & -10.85 & 17:20:53.3712 & -35:47:01.542 & 36.9 (0.1)\\
 11 & UCHII-OH4 & -10.70 & 17:20:53.3662 & -35:47:01.944 & 0.752 (0.008)\\
 12 & UCHII-OH4 & -10.70 & 17:20:53.3712 & -35:47:01.538 & 14.1 (0.1)\\
 13 & UCHII-OH6 & -10.70 & 17:20:53.3976 & -35:47:00.777 & 0.473 (0.008)\\
 14 & UCHII-OH7 & -10.70 & 17:20:53.4604 & -35:47:00.505 & 0.107 (0.008)\\
 15 & UCHII-OH7 & -10.55 & 17:20:53.4595 & -35:47:00.441 & 0.448 (0.037)\\
 16 & UCHII-OH6 & -10.55 & 17:20:53.3946 & -35:47:00.764 & 2.05 (0.04)\\
 17 & UCHII-OH4 & -10.55 & 17:20:53.3627 & -35:47:02.032 & 1.75 (0.04)\\
 18 & UCHII-OH4 & -10.55 & 17:20:53.3709 & -35:47:01.538 & 35.7 (0.1)\\
 19 & UCHII-OH4 & -10.40 & 17:20:53.3568 & -35:47:02.070 & 0.940 (0.019)\\
 20 & UCHII-OH4 & -10.40 & 17:20:53.3709 & -35:47:01.527 & 182 (1)\\
 21 & UCHII-OH6 & -10.40 & 17:20:53.3976 & -35:47:00.796 & 4.98 (0.02)\\
 22 & UCHII-OH7 & -10.40 & 17:20:53.4588 & -35:47:00.477 & 0.356 (0.019)\\
 23 & UCHII-OH6 & -10.25 & 17:20:53.3987 & -35:47:00.800 & 11.3 (0.1)\\
 24 & UCHII-OH4 & -10.25 & 17:20:53.3483 & -35:47:02.225 & 0.767 (0.105)\\
 25 & UCHII-OH4 & -10.25 & 17:20:53.3709 & -35:47:01.523 & 299 (1)\\
 26 & UCHII-OH4 & -10.10 & 17:20:53.3514 & -35:47:02.225 & 1.07 (0.05)\\
 27 & UCHII-OH4 & -10.10 & 17:20:53.3710 & -35:47:01.521 & 145 (1)\\
 28 & UCHII-OH6 & -10.10 & 17:20:53.3941 & -35:47:00.852 & 10.0 (0.1)\\
 29 & UCHII-OH6 &  -9.95 & 17:20:53.3876 & -35:47:00.953 & 7.16 (0.04)\\
 30 & UCHII-OH7 &  -9.95 & 17:20:53.4510 & -35:47:00.617 & 1.57 (0.04)\\
 31 & UCHII-OH4 &  -9.95 & 17:20:53.3531 & -35:47:02.241 & 0.966 (0.044)\\
 32 & UCHII-OH4 &  -9.95 & 17:20:53.3711 & -35:47:01.506 & 5.75 (0.04)\\
 33 & UCHII-OH7 &  -9.80 & 17:20:53.4505 & -35:47:00.634 & 3.72 (0.01)\\
 34 & UCHII-OH5 &  -9.80 & 17:20:53.4320 & -35:47:01.429 & 0.119 (0.005)\\
 35 & UCHII-OH4 &  -9.80 & 17:20:53.3516 & -35:47:02.281 & 0.486 (0.005)\\
 36 & UCHII-OH6 &  -9.80 & 17:20:53.3872 & -35:47:00.970 & 1.29 (0.01)\\
 37 & UCHII-OH4 &  -9.65 & 17:20:53.3513 & -35:47:02.265 & 0.0576 (0.0029)\\
 38 & UCHII-OH4 &  -9.65 & 17:20:53.3719 & -35:47:01.565 & 0.220 (0.003)\\
 39 & UCHII-OH6 &  -9.65 & 17:20:53.4024 & -35:47:00.490 & 0.0461 (0.0029)\\
 40 & UCHII-OH5 &  -9.65 & 17:20:53.4326 & -35:47:01.419 & 0.0999 (0.0029)\\
 41 & UCHII-OH7 &  -9.65 & 17:20:53.4513 & -35:47:00.612 & 2.54 (0.01)\\
 42 & UCHII-OH6 &  -9.50 & 17:20:53.4028 & -35:47:00.666 & 0.424 (0.003)\\
 43 & UCHII-OH4 &  -9.50 & 17:20:53.3735 & -35:47:01.604 & 0.167 (0.003)\\
 44 & UCHII-OH2 &  -9.50 & 17:20:53.3986 & -35:47:02.772 & 0.156 (0.003)\\
 45 & UCHII-OH5 &  -9.50 & 17:20:53.4333 & -35:47:01.445 & 0.148 (0.003)\\
 46 & UCHII-OH7 &  -9.50 & 17:20:53.4523 & -35:47:00.584 & 0.654 (0.003)\\
 47 & UCHII-OH5 &  -9.35 & 17:20:53.4335 & -35:47:01.448 & 0.196 (0.003)\\
 48 & UCHII-OH6 &  -9.35 & 17:20:53.4032 & -35:47:00.668 & 1.44 (0.01)\\
 49 & UCHII-OH7 &  -9.35 & 17:20:53.4517 & -35:47:00.565 & 0.124 (0.003)\\
 50 & UCHII-OH4 &  -9.35 & 17:20:53.3716 & -35:47:01.540 & 0.103 (0.003)\\
 51 & UCHII-OH2 &  -9.35 & 17:20:53.3989 & -35:47:02.770 & 0.519 (0.003)\\
 52 & UCHII-OH5 &  -9.20 & 17:20:53.4370 & -35:47:01.414 & 0.167 (0.003)\\
 53 & UCHII-OH6 &  -9.20 & 17:20:53.4034 & -35:47:00.671 & 0.987 (0.003)\\
 54 & UCHII-OH4 &  -9.20 & 17:20:53.3701 & -35:47:01.484 & 0.0554 (0.0027)\\
 55 & UCHII-OH2 &  -9.20 & 17:20:53.3992 & -35:47:02.761 & 0.402 (0.003)\\
 56 & UCHII-OH4 &  -9.05 & 17:20:53.3707 & -35:47:01.480 & 0.0391 (0.0025)\\
 57 & UCHII-OH2 &  -9.05 & 17:20:53.4027 & -35:47:02.692 & 0.101 (0.003)\\
 58 & UCHII-OH6 &  -9.05 & 17:20:53.4049 & -35:47:00.661 & 0.116 (0.003)\\
 59 & UCHII-OH5 &  -9.05 & 17:20:53.4377 & -35:47:01.453 & 0.379 (0.003)\\
 60 & UCHII-OH6 &  -8.90 & 17:20:53.4069 & -35:47:00.643 & 0.0956 (0.0027)\\
 61 & UCHII-OH2 &  -8.90 & 17:20:53.4114 & -35:47:02.644 & 0.377 (0.003)\\
 62 & UCHII-OH5 &  -8.90 & 17:20:53.4342 & -35:47:01.527 & 1.64 (0.01)\\
 63 & UCHII-OH3 &  -8.75 & 17:20:53.4174 & -35:47:01.922 & 0.631 (0.003)\\
 64 & UCHII-OH6 &  -8.75 & 17:20:53.4071 & -35:47:00.616 & 0.155 (0.003)\\
 65 & UCHII-OH2 &  -8.75 & 17:20:53.4119 & -35:47:02.631 & 1.07 (0.01)\\
 66 & UCHII-OH2 &  -8.75 & 17:20:53.4162 & -35:47:02.899 & 0.325 (0.003)\\
 67 & UCHII-OH5 &  -8.75 & 17:20:53.4341 & -35:47:01.512 & 3.32 (0.01)\\
 68 & UCHII-OH2 &  -8.60 & 17:20:53.4178 & -35:47:02.984 & 0.427 (0.003)\\
 69 & UCHII-OH5 &  -8.60 & 17:20:53.4343 & -35:47:01.474 & 3.42 (0.01)\\
 70 & UCHII-OH3 &  -8.60 & 17:20:53.4170 & -35:47:01.924 & 3.26 (0.01)\\
 71 & UCHII-OH2 &  -8.60 & 17:20:53.4128 & -35:47:02.671 & 1.55 (0.01)\\
 72 & UCHII-OH6 &  -8.60 & 17:20:53.4059 & -35:47:00.752 & 0.181 (0.003)\\
 73 & CM2-OH1-1 &  -8.60 & 17:20:53.3860 & -35:46:55.499 & 0.0580 (0.0034)\\
 74 & CM2-OH1-1 &  -8.45 & 17:20:53.3857 & -35:46:55.512 & 0.0686 (0.0034)\\
 75 & UCHII-OH6 &  -8.45 & 17:20:53.4023 & -35:47:00.894 & 0.143 (0.003)\\
 76 & UCHII-OH2 &  -8.45 & 17:20:53.4132 & -35:47:02.673 & 1.76 (0.01)\\
 77 & UCHII-OH3 &  -8.45 & 17:20:53.4168 & -35:47:01.926 & 3.24 (0.01)\\
 78 & UCHII-OH5 &  -8.45 & 17:20:53.4225 & -35:47:01.373 & 0.431 (0.003)\\
 79 & UCHII-OH1 &  -8.45 & 17:20:53.4231 & -35:47:03.199 & 0.220 (0.003)\\
 80 & UCHII-OH5 &  -8.45 & 17:20:53.4347 & -35:47:01.453 & 2.34 (0.01)\\
 81 & UCHII-OH5 &  -8.30 & 17:20:53.4349 & -35:47:01.417 & 1.62 (0.01)\\
 82 & UCHII-OH1 &  -8.30 & 17:20:53.4234 & -35:47:03.264 & 0.221 (0.003)\\
 83 & UCHII-OH5 &  -8.30 & 17:20:53.4211 & -35:47:01.390 & 0.931 (0.003)\\
 84 & CM2-OH1-1 &  -8.30 & 17:20:53.3844 & -35:46:55.576 & 0.0568 (0.0031)\\
 85 & UCHII-OH2 &  -8.30 & 17:20:53.4131 & -35:47:02.646 & 1.33 (0.01)\\
 86 & UCHII-OH6 &  -8.30 & 17:20:53.4013 & -35:47:00.896 & 0.0937 (0.0031)\\
 87 & UCHII-OH3 &  -8.30 & 17:20:53.4168 & -35:47:01.918 & 0.589 (0.003)\\
 88 & UCHII-OH1 &  -8.15 & 17:20:53.4256 & -35:47:03.297 & 0.0838 (0.0033)\\
 89 & UCHII-OH7 &  -8.15 & 17:20:53.4936 & -35:47:00.319 & 0.0679 (0.0033)\\
 90 & UCHII-OH5 &  -8.15 & 17:20:53.4352 & -35:47:01.402 & 1.15 (0.01)\\
 91 & UCHII-OH5 &  -8.15 & 17:20:53.4207 & -35:47:01.389 & 0.764 (0.003)\\
 92 & CM2-OH1-1 &  -8.15 & 17:20:53.3766 & -35:46:55.637 & 1.04 (0.01)\\
 93 & UCHII-OH6 &  -8.15 & 17:20:53.4001 & -35:47:01.002 & 0.200 (0.003)\\
 94 & CM2-OH1-1 &  -8.15 & 17:20:53.3930 & -35:46:55.610 & 0.205 (0.003)\\
 95 & UCHII-OH2 &  -8.15 & 17:20:53.4132 & -35:47:02.661 & 0.346 (0.003)\\
 96 & CM2-OH1-1 &  -8.00 & 17:20:53.3765 & -35:46:55.638 & 6.55 (0.01)\\
 97 & CM2-OH1-1 &  -8.00 & 17:20:53.3931 & -35:46:55.620 & 1.23 (0.01)\\
 98 & UCHII-OH5 &  -8.00 & 17:20:53.4126 & -35:47:01.291 & 0.344 (0.003)\\
 99 & UCHII-OH2 &  -8.00 & 17:20:53.4150 & -35:47:02.645 & 0.679 (0.003)\\
100 & UCHII-OH1 &  -8.00 & 17:20:53.4303 & -35:47:03.408 & 0.192 (0.003)\\
101 & UCHII-OH5 &  -8.00 & 17:20:53.4330 & -35:47:01.429 & 0.623 (0.003)\\
102 & UCHII-OH7 &  -8.00 & 17:20:53.4932 & -35:47:00.354 & 0.0693 (0.0033)\\
103 & UCHII-OH1 &  -7.85 & 17:20:53.4306 & -35:47:03.419 & 0.397 (0.003)\\
104 & UCHII-OH5 &  -7.85 & 17:20:53.4219 & -35:47:01.406 & 0.659 (0.003)\\
105 & UCHII-OH2 &  -7.85 & 17:20:53.4150 & -35:47:02.652 & 1.40 (0.01)\\
106 & CM2-OH1-1 &  -7.85 & 17:20:53.3922 & -35:46:55.612 & 2.38 (0.01)\\
107 & CM2-OH1-1 &  -7.85 & 17:20:53.3765 & -35:46:55.638 & 7.97 (0.01)\\
108 & CM2-OH1-1 &  -7.70 & 17:20:53.3774 & -35:46:55.623 & 5.88 (0.01)\\
109 & CM2-OH1-1 &  -7.70 & 17:20:53.3912 & -35:46:55.595 & 2.27 (0.01)\\
110 & UCHII-OH2 &  -7.70 & 17:20:53.4144 & -35:47:02.625 & 0.941 (0.004)\\
111 & UCHII-OH5 &  -7.70 & 17:20:53.4202 & -35:47:01.428 & 0.242 (0.004)\\
112 & UCHII-OH1 &  -7.70 & 17:20:53.4301 & -35:47:03.413 & 0.337 (0.004)\\
113 & UCHII-OH1 &  -7.55 & 17:20:53.4269 & -35:47:03.375 & 0.264 (0.004)\\
114 & UCHII-OH2 &  -7.55 & 17:20:53.4142 & -35:47:02.624 & 1.89 (0.01)\\
115 & CM2-OH1-1 &  -7.55 & 17:20:53.3920 & -35:46:55.605 & 0.957 (0.004)\\
116 & CM2-OH1-1 &  -7.55 & 17:20:53.3792 & -35:46:55.598 & 6.04 (0.01)\\
117 & CM2-OH1-1 &  -7.40 & 17:20:53.3796 & -35:46:55.593 & 4.08 (0.01)\\
118 & CM2-OH1-1 &  -7.40 & 17:20:53.3932 & -35:46:55.647 & 0.298 (0.003)\\
119 & UCHII-OH2 &  -7.40 & 17:20:53.4145 & -35:47:02.642 & 4.62 (0.01)\\
120 & UCHII-OH1 &  -7.40 & 17:20:53.4200 & -35:47:03.354 & 0.274 (0.003)\\
121 & UCHII-OH7 &  -7.40 & 17:20:53.4795 & -35:47:00.509 & 0.0854 (0.0032)\\
122 & UCHII-OH7 &  -7.25 & 17:20:53.4795 & -35:47:00.495 & 0.0354 (0.0026)\\
123 & UCHII-OH1 &  -7.25 & 17:20:53.4186 & -35:47:03.397 & 0.178 (0.003)\\
124 & CM2-OH1-1 &  -7.25 & 17:20:53.3832 & -35:46:55.608 & 0.630 (0.003)\\
125 & UCHII-OH2 &  -7.25 & 17:20:53.4147 & -35:47:02.648 & 2.93 (0.01)\\
126 & CM2-OH1-1 &  -7.10 & 17:20:53.3955 & -35:46:55.635 & 0.231 (0.003)\\
127 & UCHII-OH2 &  -7.10 & 17:20:53.4146 & -35:47:02.648 & 0.184 (0.003)\\
128 & UCHII-OH1 &  -7.10 & 17:20:53.4223 & -35:47:03.409 & 0.0787 (0.0027)\\
129 & CM2-OH1-1 &  -6.95 & 17:20:53.3952 & -35:46:55.630 & 0.523 (0.003)\\
130 & UCHII-OH1 &  -6.95 & 17:20:53.4265 & -35:47:03.359 & 0.209 (0.003)\\
131 & CM2-OH1-1 &  -6.80 & 17:20:53.3954 & -35:46:55.626 & 0.706 (0.003)\\
132 & UCHII-OH1 &  -6.80 & 17:20:53.4268 & -35:47:03.331 & 0.448 (0.003)\\
133 & CM2-OH1-1 &  -6.65 & 17:20:53.3953 & -35:46:55.628 & 0.235 (0.003)\\
134 & UCHII-OH1 &  -6.65 & 17:20:53.4266 & -35:47:03.313 & 0.507 (0.003)\\
135 & UCHII-OH1 &  -6.50 & 17:20:53.4261 & -35:47:03.299 & 0.456 (0.002)\\
136 & UCHII-OH1 &  -6.35 & 17:20:53.4269 & -35:47:03.312 & 0.0836 (0.0025)\\
137 & UCHII-OH7 &  -5.30 & 17:20:53.4345 & -35:47:00.355 & 0.400 (0.002)\\
138 & UCHII-OH7 &  -5.15 & 17:20:53.4346 & -35:47:00.359 & 0.904 (0.003)\\
139 & UCHII-OH7 &  -5.00 & 17:20:53.4346 & -35:47:00.349 & 0.183 (0.003)\\


==> oh_6035RRtable.tex <==
  1 & UCHII-OH4 & -12.05 & 17:20:53.3731 & -35:47:01.504 & 0.0391 (0.0023)\\
  2 & UCHII-OH4 & -11.90 & 17:20:53.3723 & -35:47:01.565 & 0.0624 (0.0025)\\
  3 & UCHII-OH4 & -11.75 & 17:20:53.3718 & -35:47:01.597 & 0.0718 (0.0025)\\
  4 & UCHII-OH4 & -11.45 & 17:20:53.3644 & -35:47:01.856 & 0.617 (0.004)\\
  5 & UCHII-OH4 & -11.45 & 17:20:53.3713 & -35:47:01.539 & 2.03 (0.01)\\
  6 & UCHII-OH4 & -11.30 & 17:20:53.3643 & -35:47:01.870 & 1.78 (0.01)\\
  7 & UCHII-OH4 & -11.30 & 17:20:53.3712 & -35:47:01.541 & 17.5 (0.1)\\
  8 & UCHII-OH4 & -11.15 & 17:20:53.3712 & -35:47:01.540 & 31.2 (0.1)\\
  9 & UCHII-OH4 & -11.15 & 17:20:53.3662 & -35:47:01.899 & 0.773 (0.018)\\
 10 & UCHII-OH4 & -11.00 & 17:20:53.3671 & -35:47:01.929 & 0.727 (0.007)\\
 11 & UCHII-OH4 & -11.00 & 17:20:53.3712 & -35:47:01.538 & 15.8 (0.1)\\
 12 & UCHII-OH4 & -10.85 & 17:20:53.3657 & -35:47:01.961 & 2.33 (0.02)\\
 13 & UCHII-OH4 & -10.85 & 17:20:53.3709 & -35:47:01.533 & 21.2 (0.1)\\
 14 & UCHII-OH4 & -10.70 & 17:20:53.3709 & -35:47:01.530 & 119 (1)\\
 15 & UCHII-OH4 & -10.55 & 17:20:53.3709 & -35:47:01.525 & 237 (1)\\
 16 & UCHII-OH7 & -10.40 & 17:20:53.4584 & -35:47:00.442 & 0.341 (0.012)\\
 17 & UCHII-OH6 & -10.40 & 17:20:53.3979 & -35:47:00.835 & 0.870 (0.012)\\
 18 & UCHII-OH4 & -10.40 & 17:20:53.3709 & -35:47:01.523 & 145 (1)\\
 19 & UCHII-OH4 & -10.40 & 17:20:53.3521 & -35:47:02.287 & 0.665 (0.012)\\
 20 & UCHII-OH4 & -10.25 & 17:20:53.3516 & -35:47:02.243 & 0.885 (0.037)\\
 21 & UCHII-OH4 & -10.25 & 17:20:53.3708 & -35:47:01.520 & 13.1 (0.1)\\
 22 & UCHII-OH6 & -10.25 & 17:20:53.3963 & -35:47:00.790 & 3.50 (0.04)\\
 23 & UCHII-OH7 & -10.25 & 17:20:53.4588 & -35:47:00.464 & 0.577 (0.037)\\
 24 & UCHII-OH4 & -10.10 & 17:20:53.3500 & -35:47:02.291 & 0.622 (0.009)\\
 25 & UCHII-OH6 & -10.10 & 17:20:53.3969 & -35:47:00.794 & 9.30 (0.01)\\
 26 & UCHII-OH7 & -10.10 & 17:20:53.4585 & -35:47:00.515 & 0.405 (0.009)\\
 27 & UCHII-OH4 &  -9.95 & 17:20:53.3494 & -35:47:02.300 & 0.156 (0.007)\\
 28 & UCHII-OH4 &  -9.95 & 17:20:53.3678 & -35:47:01.600 & 0.254 (0.007)\\
 29 & UCHII-OH6 &  -9.95 & 17:20:53.3867 & -35:47:00.963 & 3.75 (0.01)\\
 30 & UCHII-OH6 &  -9.95 & 17:20:53.3972 & -35:47:00.796 & 11.5 (0.1)\\
 31 & UCHII-OH7 &  -9.95 & 17:20:53.4583 & -35:47:00.541 & 0.319 (0.007)\\
 32 & UCHII-OH7 &  -9.80 & 17:20:53.4529 & -35:47:00.605 & 0.487 (0.006)\\
 33 & UCHII-OH5 &  -9.80 & 17:20:53.4346 & -35:47:01.470 & 0.153 (0.006)\\
 34 & UCHII-OH6 &  -9.80 & 17:20:53.3971 & -35:47:00.803 & 3.21 (0.01)\\
 35 & UCHII-OH6 &  -9.80 & 17:20:53.3866 & -35:47:00.965 & 6.13 (0.01)\\
 36 & UCHII-OH4 &  -9.65 & 17:20:53.3753 & -35:47:01.537 & 0.113 (0.004)\\
 37 & UCHII-OH6 &  -9.65 & 17:20:53.3871 & -35:47:00.954 & 1.43 (0.01)\\
 38 & UCHII-OH2 &  -9.65 & 17:20:53.3982 & -35:47:02.739 & 0.131 (0.004)\\
 39 & UCHII-OH5 &  -9.65 & 17:20:53.4340 & -35:47:01.454 & 0.217 (0.004)\\
 40 & UCHII-OH7 &  -9.65 & 17:20:53.4505 & -35:47:00.634 & 2.30 (0.01)\\
 41 & UCHII-OH4 &  -9.50 & 17:20:53.3720 & -35:47:01.616 & 0.0365 (0.0036)\\
 42 & UCHII-OH2 &  -9.50 & 17:20:53.3986 & -35:47:02.758 & 0.434 (0.004)\\
 43 & UCHII-OH6 &  -9.50 & 17:20:53.4033 & -35:47:00.618 & 0.125 (0.004)\\
 44 & UCHII-OH5 &  -9.50 & 17:20:53.4345 & -35:47:01.410 & 0.148 (0.004)\\
 45 & UCHII-OH7 &  -9.50 & 17:20:53.4510 & -35:47:00.619 & 3.86 (0.01)\\
 46 & UCHII-OH5 &  -9.35 & 17:20:53.4342 & -35:47:01.455 & 0.146 (0.003)\\
 47 & UCHII-OH6 &  -9.35 & 17:20:53.4031 & -35:47:00.666 & 1.01 (0.01)\\
 48 & UCHII-OH7 &  -9.35 & 17:20:53.4519 & -35:47:00.599 & 2.02 (0.01)\\
 49 & UCHII-OH4 &  -9.35 & 17:20:53.3742 & -35:47:01.478 & 0.0409 (0.0030)\\
 50 & UCHII-OH2 &  -9.35 & 17:20:53.3998 & -35:47:02.763 & 0.418 (0.003)\\
 51 & UCHII-OH6 &  -9.20 & 17:20:53.4033 & -35:47:00.668 & 1.97 (0.01)\\
 52 & UCHII-OH2 &  -9.20 & 17:20:53.4091 & -35:47:02.659 & 0.274 (0.004)\\
 53 & UCHII-OH5 &  -9.20 & 17:20:53.4338 & -35:47:01.534 & 0.870 (0.004)\\
 54 & UCHII-OH7 &  -9.20 & 17:20:53.4520 & -35:47:00.590 & 0.398 (0.004)\\
 55 & UCHII-OH7 &  -9.05 & 17:20:53.4484 & -35:47:00.692 & 0.0888 (0.0031)\\
 56 & UCHII-OH5 &  -9.05 & 17:20:53.4339 & -35:47:01.530 & 2.26 (0.01)\\
 57 & UCHII-OH6 &  -9.05 & 17:20:53.4035 & -35:47:00.666 & 0.759 (0.003)\\
 58 & UCHII-OH2 &  -9.05 & 17:20:53.4124 & -35:47:02.664 & 1.03 (0.01)\\
 59 & UCHII-OH6 &  -8.90 & 17:20:53.4053 & -35:47:00.689 & 0.145 (0.003)\\
 60 & UCHII-OH2 &  -8.90 & 17:20:53.4119 & -35:47:02.591 & 1.02 (0.01)\\
 61 & UCHII-OH2 &  -8.90 & 17:20:53.4156 & -35:47:02.870 & 0.812 (0.003)\\
 62 & UCHII-OH3 &  -8.90 & 17:20:53.4178 & -35:47:01.907 & 1.08 (0.01)\\
 63 & UCHII-OH5 &  -8.90 & 17:20:53.4347 & -35:47:01.485 & 2.67 (0.01)\\
 64 & UCHII-OH1 &  -8.75 & 17:20:53.4203 & -35:47:03.124 & 0.288 (0.003)\\
 65 & UCHII-OH3 &  -8.75 & 17:20:53.4169 & -35:47:01.925 & 3.50 (0.01)\\
 66 & UCHII-OH5 &  -8.75 & 17:20:53.4347 & -35:47:01.455 & 2.67 (0.01)\\
 67 & UCHII-OH6 &  -8.75 & 17:20:53.4050 & -35:47:00.755 & 0.254 (0.003)\\
 68 & UCHII-OH2 &  -8.75 & 17:20:53.4132 & -35:47:02.665 & 2.13 (0.01)\\
 69 & UCHII-OH6 &  -8.60 & 17:20:53.4062 & -35:47:00.729 & 0.267 (0.003)\\
 70 & UCHII-OH2 &  -8.60 & 17:20:53.4131 & -35:47:02.640 & 2.23 (0.01)\\
 71 & UCHII-OH3 &  -8.60 & 17:20:53.4169 & -35:47:01.923 & 2.39 (0.01)\\
 72 & UCHII-OH1 &  -8.60 & 17:20:53.4229 & -35:47:03.238 & 0.157 (0.003)\\
 73 & UCHII-OH5 &  -8.60 & 17:20:53.4347 & -35:47:01.429 & 2.16 (0.01)\\
 74 & CM2-OH-1 &  -8.45 & 17:20:53.3853 & -35:46:55.530 & 0.0536 (0.0029)\\
 75 & UCHII-OH6 &  -8.45 & 17:20:53.4046 & -35:47:00.814 & 0.271 (0.003)\\
 76 & UCHII-OH2 &  -8.45 & 17:20:53.4134 & -35:47:02.653 & 0.639 (0.003)\\
 77 & UCHII-OH3 &  -8.45 & 17:20:53.4153 & -35:47:01.855 & 0.147 (0.003)\\
 78 & UCHII-OH5 &  -8.45 & 17:20:53.4353 & -35:47:01.399 & 1.85 (0.01)\\
 79 & UCHII-OH7 &  -8.45 & 17:20:53.4964 & -35:47:00.195 & 0.0287 (0.0029)\\
 80 & UCHII-OH7 &  -8.30 & 17:20:53.4944 & -35:47:00.300 & 0.0788 (0.0028)\\
 81 & UCHII-OH2 &  -8.30 & 17:20:53.4148 & -35:47:02.655 & 0.396 (0.003)\\
 82 & UCHII-OH5 &  -8.30 & 17:20:53.4344 & -35:47:01.405 & 1.22 (0.01)\\
 83 & CM2-OH-1 &  -8.30 & 17:20:53.3856 & -35:46:55.539 & 0.0726 (0.0028)\\
 84 & UCHII-OH6 &  -8.30 & 17:20:53.4053 & -35:47:01.041 & 0.339 (0.003)\\
 85 & UCHII-OH7 &  -8.15 & 17:20:53.4943 & -35:47:00.299 & 0.0483 (0.0030)\\
 86 & UCHII-OH1 &  -8.15 & 17:20:53.4288 & -35:47:03.378 & 0.0755 (0.0030)\\
 87 & UCHII-OH5 &  -8.15 & 17:20:53.4212 & -35:47:01.403 & 0.788 (0.003)\\
 88 & UCHII-OH5 &  -8.15 & 17:20:53.4354 & -35:47:01.418 & 0.373 (0.003)\\
 89 & UCHII-OH6 &  -8.15 & 17:20:53.4024 & -35:47:00.944 & 0.129 (0.003)\\
 90 & CM2-OH-1 &  -8.15 & 17:20:53.3923 & -35:46:55.583 & 0.0745 (0.0030)\\
 91 & CM2-OH-1 &  -8.15 & 17:20:53.3775 & -35:46:55.610 & 0.173 (0.003)\\
 92 & UCHII-OH2 &  -8.15 & 17:20:53.4150 & -35:47:02.655 & 1.28 (0.01)\\
 93 & CM2-OH-1 &  -8.00 & 17:20:53.3763 & -35:46:55.641 & 3.71 (0.01)\\
 94 & CM2-OH-1 &  -8.00 & 17:20:53.3931 & -35:46:55.621 & 0.770 (0.003)\\
 95 & UCHII-OH2 &  -8.00 & 17:20:53.4148 & -35:47:02.648 & 1.31 (0.01)\\
 96 & UCHII-OH5 &  -8.00 & 17:20:53.4216 & -35:47:01.403 & 0.885 (0.003)\\
 97 & UCHII-OH1 &  -8.00 & 17:20:53.4305 & -35:47:03.422 & 0.216 (0.003)\\
 98 & UCHII-OH1 &  -7.85 & 17:20:53.4302 & -35:47:03.409 & 0.232 (0.004)\\
 99 & UCHII-OH2 &  -7.85 & 17:20:53.4141 & -35:47:02.629 & 2.04 (0.01)\\
100 & UCHII-OH5 &  -7.85 & 17:20:53.4203 & -35:47:01.429 & 0.315 (0.004)\\
101 & CM2-OH-1 &  -7.85 & 17:20:53.3763 & -35:46:55.641 & 10.6 (0.1)\\
102 & CM2-OH-1 &  -7.85 & 17:20:53.3924 & -35:46:55.619 & 2.18 (0.01)\\
103 & CM2-OH-1 &  -7.70 & 17:20:53.3765 & -35:46:55.636 & 8.96 (0.01)\\
104 & CM2-OH-1 &  -7.70 & 17:20:53.3904 & -35:46:55.599 & 2.28 (0.01)\\
105 & UCHII-OH2 &  -7.70 & 17:20:53.4145 & -35:47:02.638 & 4.75 (0.01)\\
106 & UCHII-OH5 &  -7.70 & 17:20:53.4192 & -35:47:01.422 & 0.300 (0.004)\\
107 & UCHII-OH1 &  -7.70 & 17:20:53.4280 & -35:47:03.313 & 0.173 (0.004)\\
108 & CM2-OH-1 &  -7.55 & 17:20:53.3783 & -35:46:55.610 & 6.10 (0.01)\\
109 & UCHII-OH2 &  -7.55 & 17:20:53.4147 & -35:47:02.645 & 3.19 (0.01)\\
110 & UCHII-OH5 &  -7.55 & 17:20:53.4185 & -35:47:01.434 & 0.113 (0.004)\\
111 & UCHII-OH1 &  -7.55 & 17:20:53.4245 & -35:47:03.365 & 0.156 (0.004)\\
112 & CM2-OH-1 &  -7.55 & 17:20:53.3887 & -35:46:55.578 & 1.20 (0.01)\\
113 & UCHII-OH7 &  -7.40 & 17:20:53.4800 & -35:47:00.511 & 0.0476 (0.0033)\\
114 & CM2-OH-1 &  -7.40 & 17:20:53.3799 & -35:46:55.594 & 5.15 (0.01)\\
115 & UCHII-OH2 &  -7.40 & 17:20:53.4146 & -35:47:02.638 & 0.222 (0.003)\\
116 & UCHII-OH1 &  -7.40 & 17:20:53.4182 & -35:47:03.378 & 0.281 (0.003)\\
117 & UCHII-OH7 &  -7.25 & 17:20:53.4800 & -35:47:00.545 & 0.0917 (0.0025)\\
118 & UCHII-OH1 &  -7.25 & 17:20:53.4211 & -35:47:03.363 & 0.298 (0.002)\\
119 & CM2-OH-1 &  -7.25 & 17:20:53.3799 & -35:46:55.595 & 1.42 (0.01)\\
120 & UCHII-OH1 &  -7.10 & 17:20:53.4258 & -35:47:03.309 & 0.412 (0.003)\\
121 & UCHII-OH7 &  -7.10 & 17:20:53.4792 & -35:47:00.515 & 0.0714 (0.0026)\\
122 & CM2-OH-1 &  -6.95 & 17:20:53.3938 & -35:46:55.644 & 0.122 (0.003)\\
123 & UCHII-OH1 &  -6.95 & 17:20:53.4260 & -35:47:03.306 & 0.549 (0.003)\\
124 & CM2-OH-1 &  -6.80 & 17:20:53.3952 & -35:46:55.628 & 0.366 (0.002)\\
125 & UCHII-OH1 &  -6.80 & 17:20:53.4261 & -35:47:03.300 & 0.537 (0.002)\\
126 & UCHII-OH1 &  -6.65 & 17:20:53.4269 & -35:47:03.321 & 0.107 (0.003)\\
127 & CM2-OH-1 &  -6.65 & 17:20:53.3955 & -35:46:55.627 & 0.765 (0.003)\\
128 & CM2-OH-1 &  -6.50 & 17:20:53.3956 & -35:46:55.626 & 0.461 (0.003)\\
129 & CM2-OH-1 &  -6.35 & 17:20:53.3959 & -35:46:55.690 & 0.0338 (0.0028)\\
130 & UCHII-OH1 &  -6.05 & 17:20:53.4562 & -35:47:03.778 & 0.0325 (0.0026)\\
131 & UCHII-OH1 &  -5.90 & 17:20:53.4540 & -35:47:03.738 & 0.0254 (0.0025)\\
132 & UCHII-OH7 &  -5.30 & 17:20:53.4346 & -35:47:00.356 & 0.186 (0.002)\\
133 & UCHII-OH7 &  -5.15 & 17:20:53.4346 & -35:47:00.357 & 0.930 (0.003)\\
134 & UCHII-OH7 &  -5.00 & 17:20:53.4345 & -35:47:00.359 & 0.497 (0.003)\\
135 & UCHII-OH7 &  -4.85 & 17:20:53.4369 & -35:47:00.380 & -0.0219 (-0.0025)\\

